Enhanced Modeling of Contingency Response in Security-constrained Optimal Power Flow

This paper provides an enhanced modeling of the contingency response that collectively reflects high-fidelity physical and operational characteristics of power grids. Integrating active and reactive power contingency responses into the security-constrained optimal power flow (SCOPF) problem is challenging, due to the nonsmoothness and nonconvexity of feasible sets in consequence of piece-wise curves representing generator characteristics. We introduce a continuously-differentiable model using functions that closely resemble PV/PQ switching and the generator contingency response. These models enforce physical and operational limits by optimally allocating active power imbalances among available generators and deciding the bus type to switch from the PV type to the PQ type. The efficacy of this method is numerically validated on the IEEE 30-bus, 300-bus, and 118-bus systems with 12, 10, and 100 contingencies, respectively.

==> PV_PQ paper/abstract.tex <==
This paper provides an enhanced modeling of the contingency response that collectively reflects high-fidelity physical and operational characteristics of power grids. 
%We consider contingency scenarios involving the outage of arbitrary sets of generators and lines. 
Integrating active and reactive power contingency responses into the security-constrained optimal power flow (SCOPF) problem is challenging, due to the nonsmoothness and nonconvexity of feasible sets in consequence of piece-wise curves representing generator characteristics. We introduce a continuously-differentiable model using functions that closely resemble PV/PQ switching and the generator contingency response. These models enforce physical and operational limits by optimally allocating active power imbalances among available generators and deciding the bus type to switch from the PV type to the PQ type. The efficacy of this method is numerically validated on the IEEE 30-bus, 300-bus, and 118-bus systems with 12, 10, and 100 contingencies, respectively.  

     


% Traditional power flow algorithms assume that a slack bus is present and that the frequency is not fluctuating. In islanded systems and microgrids, however, these assumptions are not valid as such systems usually do not have a strong source performing as the slack bus and the system frequency is more prone to vary near nominal frequency. Distribution system operating environments are changing rapidly. 
%
%
%For example, with the steady and significant increase in distributed generation expected, planning and operating application techniques must also change. The single slack bus assumption is typically employed in steady-state distribution power flow solvers. Specifically, a distributed slack bus model based on the concept of generator domains will be discussed and integrated into a power flow solver. 

 


==> PV_PQ paper/casestudy.tex <==
\section{Case Studies}
Numerical studies on the IEEE 30-bus, 118-bus, and 300-bus systems demonstrate the efficacy of the continuously-differentiable SCOPF model. The main purpose is to minimize pre-contingency power generation cost while securing the post-contingency operation. The secure operation prevents physical and operational violations by means of optimally, allocating active power imbalances among available generators and deciding the type of bus, i.e., PV/PQ switching, respectively. To this end, we consider several numerical experiments on the IEEE benchmark under an extensive list of contingency scenarios, each representing the outage of randomly chosen components, e.g., generator or line. Herein, it is ensured that randomly-chosen lines do not lead to an islanding in the grid. These studies are examined on a PC with 16-core, Xeon processor, and 256 GB RAM using Artelys Knitro v12.2.2. The allowable feasibility violation is set to $10^{-6}$ for the obtained solution of given scenarios in Table~\ref{tab:1} and \ref{tab:300}. The $h$ and $k$ values used in the simulations are given and demonstrated by Figures \ref{fig:fig9} and \ref{fig:fig10}. For all of the case studies, we also simulated the continuous complementarity model from \cite{l11}, which failed to converge to a feasible point.
     
\subsection{IEEE 30-bus System with 12 Contingencies}
The IEEE benchmark considered has 30 buses connected with 41 transmission lines, 6 generators, and 20 loads. In this benchmark, bus 1 is assigned as the slack bus; buses 2, 13, 22, 23, 27 are PV buses, and the rest are PQ buses. Consider this IEEE 30-bus system under 12 contingency scenarios as described in Table~\ref{tab:1}. To maintain system reliability under certain contingencies, the benchmark data is changed by reducing the load demand in half. Hence, the solution to the OPF problem with no contingency results in a minimum generation cost of 2847.8. Considering contingency cases in Table~\ref{tab:1} using (\ref{eq:ac1}) increases the cost during normal conditions by $11.24\%$ to 3167.9. Tables~\ref{tab:2}-\ref{tab:4} represent active power, reactive power, and voltage variations of the power grid in response to given contingencies. The proposed method distributes network's active power imbalance complying with (\ref{eq:activep}), which is due to the outage of a network component, among available generators given in Table~\ref{tab:2}. It can be observed from Table~\ref{tab:2} that the outage of a transmission line, scenarios 7-12, does not cause a considerable power redispatch. Table~\ref{tab:3} and ~\ref{tab:4} represent the reactive power and voltage relations in the case of a network component outage. It is expected that the PV buses maintain their base case voltage levels during contingencies as much as their capacity limits permit. The highlighted values in \textbf{bold} in Table~\ref{tab:4} for the scenarios 1-6, refer to the PV/PQ switching due to a generator outage. It should be noted that the outage of a transmission line, for the scenarios 7-12, does not usually require PV/PQ switching except for the bus 1 as reported in Table~\ref{tab:4}. 

Table~\ref{tab:5} compares the performance of sigmoid functions, (\ref{eq:ac1})-(\ref{eq:ac5}), in terms of the objective value and required time to solve a given problem. It can be inferred that (\ref{eq:ac1}) and (\ref{eq:ac4}) offer the best approximations in terms of objective values while others, (\ref{eq:ac2}), (\ref{eq:ac3}), (\ref{eq:ac5}) successfully recover the feasible solution considering the generator response in the case of a randomly-outed component.

\begin{table}[h]
	\centering
	\caption{List of Contingencies for IEEE 30-bus system}
			\resizebox{0.6\columnwidth}{!}{
				
	\begin{tabular}{|l|c|c|}
		\hline
		\textbf{Contingency} & \textbf{Generator} & \textbf{Line} \\
		\textbf{\;\;\;\;Number} & \textbf{Number} & \textbf{Number}\\
		\hline
		\;\;\;\;\;\;\;\;\;1& 5 & - \\
		\hline
		\;\;\;\;\;\;\;\;\;2& 6 & - \\
		\hline
		\;\;\;\;\;\;\;\;\;3& 1 & - \\
		\hline
		\;\;\;\;\;\;\;\;\;4& 4 & - \\
		\hline
		\;\;\;\;\;\;\;\;\;5& 3 & - \\
		\hline
		\;\;\;\;\;\;\;\;\;6& 2 & - \\
		\hline
		\;\;\;\;\;\;\;\;\;7& - & 2\\ 
		\hline
		\;\;\;\;\;\;\;\;\;8& - & 25\\
		\hline
		\;\;\;\;\;\;\;\;\;9& - & 20\\ 
		\hline
		\;\;\;\;\;\;\;\;10& - & 35 \\
		\hline
		\;\;\;\;\;\;\;\;11& - & 9 \\ 
		\hline
		\;\;\;\;\;\;\;\;12& - & 1\\
		\hline
	\end{tabular}}
\label{tab:1}
\end{table}

\begin{table*}
	\caption{Active power variations in response to contingency scenarios (pu)}
	%	\setlength\extrarowheight{2.5pt}
	\centering
	\resizebox{2\columnwidth}{!}{
		\begin{tabular}{|l||*{13}{c|}}\hline
			\diagbox[innerwidth = 1.9cm, height = 5.8ex]{Bus Nr.}{Sc. Nr.}
			%	\backslashbox{Method}{\strut Time \\interval (s)}
			&\makebox[3em]{0}&\makebox[3em]{1}&\makebox[3em]{2}
			&\makebox[3em]{3}&\makebox[3em]{4}&\makebox[3em]{5}
			&\makebox[3em]{6}&\makebox[3em]{7}&\makebox[3em]{8}
			&\makebox[3em]{9}&\makebox[3em]{10}&\makebox[3em]{11}
			&\makebox[3em]{12}\\\hline\hline
			\;\;\;\;\;\;\;\;\;1 &0.2880  &  0.2946 &   0.2945   &      0  &  0.2894  &  0.3152  &  0.3541  &  0.2878   &  0.2875  &  0.2874  &  0.2874  &  0.2874  &  0.2875 \\\hline 
			\;\;\;\;\;\;\;\;\;2 &0.4073  &  0.4131 &   0.4130   & 0.4488   & 0.4085  &  0.4311 &        0  &  0.4072 &   0.4069  &  0.4068  &  0.4068 &   0.4068 &   0.4069 \\\hline 
 			\;\;\;\;\;\;\;\;\;22&0.1755 &   0.1788  &  0.1788  &  0.1992 &   0.1762   &      0 &   0.2086  &  0.1755  &  0.1753 &   0.1752  &  0.1752  &  0.1752  &  0.1753\\\hline 
			\;\;\;\;\;\;\;\;\;27&0.0077 &   0.0208 &   0.0206  &  0.0850   &      0  &  0.0528&   0.1152 &   0.0109 &   0.0105  &  0.0102  &  0.0103 &   0.0103  &  0.0105 \\\hline 
			\;\;\;\;\;\;\;\;\;23&0.0386 &       0  &  0.0484 &   0.1096  &  0.0408  &  0.0794  &  0.1376 &   0.0385 &  0.0381 &   0.0379  &  0.0379  &  0.0379 &   0.0381 \\\hline
			\;\;\;\;\;\;\;\;\;13&0.0375 &   0.0478   &      0  &  0.1085 &   0.0401 &   0.0783   & 0.1365  &  0.0378 &  0.0374  &  0.0371 &   0.0371  &  0.0371 &   0.0374 \\\hline
	\end{tabular}}
	\label{tab:2}
\end{table*}

\begin{table*}
	\caption{Reactive power variations in response to contingency scenarios (pu)}
	%	\setlength\extrarowheight{2.5pt}
	\centering
	\resizebox{2\columnwidth}{!}{
		\begin{tabular}{|l||*{13}{c|}}\hline
			\diagbox[innerwidth = 1.9cm, height = 5.8ex]{Bus Nr.}{Sc. Nr.}
			%	\backslashbox{Method}{\strut Time \\interval (s)}
			&\makebox[3em]{0}&\makebox[3em]{1}&\makebox[3em]{2}
			&\makebox[3em]{3}&\makebox[3em]{4}&\makebox[3em]{5}
			&\makebox[3em]{6}&\makebox[3em]{7}&\makebox[3em]{8}
			&\makebox[3em]{9}&\makebox[3em]{10}&\makebox[3em]{11}
			&\makebox[3em]{12}\\\hline\hline
			\;\;\;\;\;\;\;\;\;1 & -0.0888  & -0.0298  & -0.0216   &      0  & -0.0257  & -0.0245 &   0.0243 &  -0.0599 &  -0.0296 &  -0.0298 &  -0.0299  & -0.0316 &  -0.0306 \\\hline 
			\;\;\;\;\;\;\;\;\;2 & 0.1016 &   0.0500 &   0.0861  &  0.0345  &  0.0743 &   0.1011 &        0  &  0.0795 &   0.0454 &   0.0463 &   0.0459 &   0.0674 &  0.0886 \\\hline 
			\;\;\;\;\;\;\;\;\;22&0.1358 &   0.1554  &  0.1736  &  0.1425 &   0.1603  &       0  &  0.1587 &   0.1447 &   0.1164  &  0.1340  &  0.1470  &  0.1301 &  0.1337\\\hline 
			\;\;\;\;\;\;\;\;\;27&0.0748  &  0.0762  &  0.0750  &  0.0604  &       0 &   0.0905  &  0.0628  &  0.0789 &   0.0729 &   0.0732  &  0.0509 &   0.0709 &   0.0728\\\hline 
			\;\;\;\;\;\;\;\;\;23&0.0356   &      0  &  0.0817 &   0.0024  &  0.0498 &   0.0812  & -0.0074  &  0.0392 &   0.0520  &  0.0361 &   0.0465 &   0.0354 &   0.0355 \\\hline
			\;\;\;\;\;\;\;\;\;13&0.1360  &  0.1450   &      0  &  0.1375  &  0.1371  &  0.1569 &   0.1443 &   0.1428 &  0.1399  &  0.1345   & 0.1339  &  0.1333  &  0.1336 \\\hline
	\end{tabular}}
	\label{tab:3}
\end{table*}

\begin{table*}
	\caption{Voltage variations in response to contingency scenarios (pu). Values in red color indicate PV/PQ switching.}
	%	\setlength\extrarowheight{2.5pt}
	\centering
	\resizebox{2\columnwidth}{!}{
		\begin{tabular}{|l||*{13}{c|}}\hline
			\diagbox[innerwidth = 1.9cm, height = 5.8ex]{Bus Nr.}{Sc. Nr.}
			%	\backslashbox{Method}{\strut Time \\interval (s)}
			&\makebox[3em]{0}&\makebox[3em]{1}&\makebox[3em]{2}
			&\makebox[3em]{3}&\makebox[3em]{4}&\makebox[3em]{5}
			&\makebox[3em]{6}&\makebox[3em]{7}&\makebox[3em]{8}
			&\makebox[3em]{9}&\makebox[3em]{10}&\makebox[3em]{11}
			&\makebox[3em]{12}\\\hline\hline
			\;\;\;\;\;\;\;\;\;1 & 1.0465  &  {\textbf{1.0489}} &   {\textbf{1.0487}}  &  1.0466 &   {\textbf{1.0488}}  &  {\textbf{1.0488}} &   {\textbf{1.0477}}  &  {\textbf{1.0500}}  &  {\textbf{1.0489}}  &  {\textbf{1.0489}} &   {\textbf{1.0489}}  &  {\textbf{1.0490}} &   {\textbf{1.0490}}\\\hline 
			\;\;\;\;\;\;\;\;\;2 & 1.0470  &  1.0470  &  1.0470 &   1.0470 &   1.0470 &  1.0470  &  {\textbf{1.0409}}  &  1.0470  &  1.0470  &  1.0470 &   1.0470 &   1.0470 &   1.0470 \\\hline 
			\;\;\;\;\;\;\;\;\;22&1.0487   & 1.0487  &  1.0487  &  1.0487  &  1.0487  &  {\textbf{1.0229}}  &  1.0487  &  1.0487 &   1.0487 &   1.0487 &   1.0487 &   1.0487 &   1.0487\\\hline 
			\;\;\;\;\;\;\;\;\;27&1.0488  &  1.0488  &  1.0488  &  1.0488  &  {\textbf{1.0272}}  &  1.0489  &  1.0489  &  1.0489  &  1.0489 &   1.0489 &   1.0489 &   1.0489 &   1.0489\\\hline 
			\;\;\;\;\;\;\;\;\;23&1.0470  & {\textbf{1.0373}}  &  1.0470  &  1.0471  &   1.0471 &   1.0470  &  1.0471 &   1.0471  &  1.0471 &   1.0471 &   1.0471 &   1.0471 &    1.0471 \\\hline
			\;\;\;\;\;\;\;\;\;13& 1.0664 &   1.0665 &   {\textbf{1.0325}} &   1.0665 &   1.0665 &   1.0665 &  1.0665 &   1.0665  &  1.0665 &   1.0665 &   1.0665 &   1.0665 &   1.0665 \\\hline
	\end{tabular}}
	\label{tab:4} 
\end{table*}

\begin{table}
	\centering
	\caption{Performance Comparison for the Proposed Functions}
	\resizebox{0.8\columnwidth}{!}{
		
		\begin{tabular}{|l|c|c|}
			\hline
			\textbf{\;\;\;\;\;Continuously-differentiable Function} & \textbf{Objective} & \textbf{Required} \\
			\textbf{} & \textbf{Value} & \textbf{Time (s)}\\
			\hline
			Inverse hyperbolic tangent (\ref{eq:ac1})& 3167.9 & 6.32 \\
			\hline
			Inverse arctangent (\ref{eq:ac2})& 3168.6 & 6.25 \\
			\hline
			Inverse algebraic (\ref{eq:ac3})& 3168.1 & 6.44 \\
			\hline
			Inverse error (\ref{eq:ac4})& 3167.8 & 6.86 \\
			\hline
			Inverse absolute value (\ref{eq:ac5})& 3169.1 & 7.60 \\
			\hline
	\end{tabular}}
	\label{tab:5}
\end{table}


\subsection{IEEE 300-bus System with 10 Contingencies}
Herein, we consider the IEEE 300-bus system with 10 randomly selected contingencies as indicated in Table~\ref{tab:300}. We used the inverse hyperbolic tangent function (\ref{eq:ac1}) with $k=1$ and $h=50$. The resulting model converged within 25 minutes. The OPF solution with no contingency results in the cost of $719725.11$, and adding contingencies increases the cost by $\%0.23$ to $721396.85$.


\begin{table}
	\centering
	\caption{List of Contingencies for IEEE 300-bus system}
	\resizebox{0.6\columnwidth}{!}{
		
		\begin{tabular}{|l|c|c|}
			\hline
			\textbf{Contingency} & \textbf{Generator} & \textbf{Line} \\
			\textbf{\;\;\;\;Number} & \textbf{Number} & \textbf{Number}\\
			\hline
			\;\;\;\;\;\;\;\;\;1& 28 & - \\
			\hline
			\;\;\;\;\;\;\;\;\;2& 52 & - \\
			\hline
			\;\;\;\;\;\;\;\;\;3& 7 & - \\
			\hline
			\;\;\;\;\;\;\;\;\;4& 19 & - \\
			\hline
			\;\;\;\;\;\;\;\;\;5& 35 & - \\
			\hline
			\;\;\;\;\;\;\;\;\;6& - & 214 \\
			\hline
			\;\;\;\;\;\;\;\;\;7& - & 301\\ 
			\hline
			\;\;\;\;\;\;\;\;\;8& - & 345\\
			\hline
			\;\;\;\;\;\;\;\;\;9& - & 241\\ 
			\hline
			\;\;\;\;\;\;\;\;10& - & 94 \\
			\hline
	\end{tabular}}
	\label{tab:300}
\end{table}

\subsection{IEEE 118-bus System with 100 Contingencies}
In this case study, the IEEE 118-bus system is considered with 100 uniformly chosen contingencies. Similar to the previous case study, the inverse hyperbolic tangent function (\ref{eq:ac1}) is used with $k=1$ and $h=50$. The resulting model converged within 18 hours. The solution of the OPF problem with no contingency results in the cost of $129660.70$, and the addition of contingencies leads to a $\%0.99$ increment in cost to $130946.79$.


%\begin{table*}[ht]
%	\caption{Wide single-column table in a twocolumn document.}
%	\centering
%	\resizebox{2\columnwidth}{!}{
%		\begin{tabular}{p{0.07\linewidth}p{0.07\linewidth}p{0.07\linewidth}p{0.07\linewidth}p{0.07\linewidth}p{0.07\linewidth}p{0.07\linewidth}p{0.07\linewidth}p{0.07\linewidth}p{0.07\linewidth}p{0.07\linewidth}p{0.07\linewidth}p{0.07\linewidth}}
%			\hline
%			Base Case & Sc. 1 & Sc. 2& Sc. 3 & Sc. 4& Sc. 5 & Sc. 6& Sc. 7 & Sc. 8& Sc. 9 & Sc. 10& Sc. 11 & Sc. 12\\
%			\hline
%			Base &  1 &  2 &  3 &  4 &  5 &  6 & 7 &  8 &  9 & 10 & 11 &  12\\
%			Base &  1 &  2 &  3 &  4 &  5 &  6 & 7 &  8 &  9 & 10 & 11 &  12\\
%			\hline
%	\end{tabular}}
%\end{table*}
%\begin{table*}[ht]
%		\caption{Wide single-column table in a twocolumn document.}
%	\centering
%\begin{tabular}{SSSSSSSS} \toprule
%	{$Bus Nr.$} & {$\Re\{\underline{\mathfrak{X}}(m)\}$} & {$-\Im\{\underline{\mathfrak{X}}(m)\}$} & {$\mathfrak{X}(m)$} & {$\frac{\mathfrak{X}(m)}{23}$} & {$A_m$} & {$\varphi(m)\ /\ ^{\circ}$} & {$\varphi_m\ /\ ^{\circ}$} \\ \midrule
%	1  & 16.128 & +8.872 & 16.128 & 1.402 & 1.373 & -146.6 & -137.6 \\
%	2  & 3.442  & -2.509 & 3.442  & 0.299 & 0.343 & 133.2  & 152.4  \\
%	3  & 1.826  & -0.363 & 1.826  & 0.159 & 0.119 & 168.5  & -161.1 \\
%	4  & 0.993  & -0.429 & 0.993  & 0.086 & 0.08  & 25.6   & 90     \\ \midrule
%	5  & 1.29   & +0.099 & 1.29   & 0.112 & 0.097 & -175.6 & -114.7 \\
%	6  & 0.483  & -0.183 & 0.483  & 0.042 & 0.063 & 22.3   & 122.5  \\
%	7  & 0.766  & -0.475 & 0.766  & 0.067 & 0.039 & 141.6  & -122   \\
%	8  & 0.624  & +0.365 & 0.624  & 0.054 & 0.04  & -35.7  & 90     \\ \midrule
%	9  & 0.641  & -0.466 & 0.641  & 0.056 & 0.045 & 133.3  & -106.3 \\
%	10 & 0.45   & +0.421 & 0.45   & 0.039 & 0.034 & -69.4  & 110.9  \\
%	11 & 0.598  & -0.597 & 0.598  & 0.052 & 0.025 & 92.3   & -109.3 \\ \bottomrule
%\end{tabular}
%\end{table*}

==> PV_PQ paper/conclusion.tex <==
\section{Conclusion}

This paper tackles the SCOPF problem that considers the piecewise-discontinuous model of generator active and reactive power contingency responses by means of several continuously-differentiable models. The proposed approach provides state and decision variables to ensure continuity of power grid operation even under contingencies. The problem is expressed as a nonlinear programming formulation and involves piecewise-smooth models due to the characteristics of the active and reactive power contingency. We replace these non-differentiable curves with several continuously-differentiable surrogates that are tractable and can be solved with various numerical solvers. The proposed models are numerically verified on several IEEE benchmarks under various contingencies.
 


==> PV_PQ paper/dsbmodel.tex <==
\section{Enhanced Modeling of a Generator Response}
To capture the nonlinear characteristics of a power system, such as PV/PQ switching and generator contingency response, and to streamline these policies, we define the following set.
\begin{definition}
For $\theta \in [0, \pi/4)$, define $\Fcal_{\theta}\subseteq \mathbb{R}^2$ as
\begin{align} 
&\Fcal_{\theta}  \triangleq\Big\{\;(x,y)\in\mathbb{R}^2\;|\;-1 \leq x \leq 1\nonumber\\
&\;\wedge\;\min\{\max\left\{0,y-\mathrm{tan}(\theta)x\},\max\{0,1-x\}\right\}=0\nonumber\\
&\;\wedge\;\min\{\max\left\{0,\mathrm{tan}(\theta)x-y\},\max\{0,1+x\}\right\}=0\;\Big\}, \label{eq:set_orig}
\end{align}
\end{definition}
\noindent where $\theta$ denotes the slope for the segment
within the interval $[-1,1]$. Herein, each pair ($x$, $y$) represents the coordinates on a piecewise-smooth curve. In the following section, we will provide a smooth version of $\Fcal_{\theta}$ in order to facilitate local search. This is illustrated in Figure \ref{fig2}.
% \begin{figure}
%	\centering
%	\includegraphics[width=\columnwidth]{figures/fig2.pdf}
%	\caption{I will plot conceptual figure for different values of $\theta$.}
%	\label{fig:fig21} 
%\end{figure}
%\begin{figure}   
%	\centering
%	\begin{subfigure}{0.48\columnwidth}
%		\centering 
%		\includegraphics[width=\linewidth]{figures/fig2_2.pdf}
%		\caption{The characteristics of a pair, $(x,y) \in \Fcal_{\theta}$, for different slope values.}
%	\end{subfigure}%
%	~
%	\begin{subfigure}{0.48\columnwidth}
%		\centering
%		\includegraphics[width=\linewidth]{figures/fig2.pdf}
%		\caption{The characteristics of a pair, $(x,y) \in \Fcal^{\mathrm{smooth}}_{\theta}$, for different slope values.}
%	\end{subfigure}%
%	\caption{The characteristics of $\Fcal_{\theta}$ and $\Fcal^{\mathrm{smooth}}_{\theta}$ when $\theta=0$, $\theta=\pi/8$, $\theta=\pi/6$, $\theta=\pi/4$.}
%\end{figure}
\begin{figure} 
	\centering
	\subfloat(a){%
		\includegraphics[width=0.40\linewidth]{figures/fig2_2.pdf}}
	\hfill
	\subfloat(b){%
		\includegraphics[width=0.40\linewidth]{figures/fig2.pdf}}
	\caption{The characteristics of (a) $(x,y) \in \Fcal_{\theta}$ and (b) $(x,y) \in \Fcal^{\mathrm{smooth}}_{\theta}$ for different slope values, $\theta=0$, $\theta=\pi/8$, $\theta=\pi/6$, $\theta=\pi/4$.}
	\label{fig2} 
\end{figure}
\subsection{Generator Active Power Contingency Response}
For now, assume that there is no limit imposed on post-contingency active power injections, i.e.,
\begin{align}
p^{\max}_{c,g} = -p^{\min}_{c,g} = \infty \qquad \forall c \in \Ccal \setminus{0}, g\in\Gcal. \label{111}
\end{align}
Given assumption (\ref{111}), the active power imbalance due to changes in network configuration, transmission losses, or load profile is distributed among operational generators as
\begin{equation}
p^{\mathrm{gen}}_{c,g}=p^{\mathrm{gen}}_{0,g}+\alpha_{c,g} \Delta_c,
\end{equation}
where 
\begin{itemize}
\item $p^{\mathrm{gen}}_{c,g}$ is the post-contingency active power produced by $g \in \Gcal$; 
\item $p^{\mathrm{gen}}_{0,g}$ is the base case active power of generator $g$; 
\item $\Delta_c$ represents the amount of post contingency redispatch; 
\item $\alpha_{c,g}$ denotes the weight of contribution to this redispatch by generator $g$. 
\end{itemize}
If a generator is operational but not selected to contribute to redispatch, it maintains its active power generation from the base case, i.e., 
\begin{align}
\alpha_{c,g}=0\quad\Rightarrow\quad p^{\mathrm{gen}}_{c,g}=p^{\mathrm{gen}}_{0,g}.
\end{align}
%Herein, if a generator is failed in the contingency, the contingency case active power generation and its contribution to redispatch will be $p^{\mathrm{gen}}_{c,g}=0$ and $\alpha_{c,g}=0$, respectively. 

In the presence of post-contingency generator active power limits (i.e., when the assumption (\ref{111}) does not hold), a generator that contributes to a given contingency can readjust its active power generation to the extent that its capacity limits permit. This behavior can be formulated using logical functions, and Min-Max operators. For every $ c \in \Ccal$ and $g \in \Gcal$, the logical functions representation of generator active power contingency response, using disjunction of linear constraints, is as follows:
 \begin{subequations}\label{eq:activep}
	%{\small{
\begin{align} 
& p^{\mathrm{gen}}_{c,g} = p^{\max}_{c,g},&&\hspace{-0.2mm}\mathrm{if}\qquad p^{\mathrm{max}}_{c,g}< p^{\mathrm{gen}}_{0,g}+\alpha_{c,g} \Delta_c, %&&&\hspace{-4.5mm} \forall c \in \Ccal, g \in \Gcal, 
\label{eq:activep2} \\
& p^{\mathrm{gen}}_{c,g} = p^{\min}_{c,g},&&\hspace{-0.2mm}\mathrm{if}\qquad p^{\mathrm{min}}_{c,g}> p^{\mathrm{gen}}_{0,g}+\alpha_{c,g} \Delta_c, %&&&\hspace{-4.5mm}  \forall c \in \Ccal, g \in \Gcal, 
\label{eq:activep3}\\
&p^{\mathrm{gen}}_{c,g}=p^{\mathrm{gen}}_{0,g}+\alpha_{c,g} \Delta_c ,&&\hspace{-6.5mm} \qquad \mathrm{otherwise} %&&&\hspace{-6.5mm} \forall c \in \Ccal, g \in \Gcal
. \label{eq:activep1}
\end{align}%}}
\end{subequations}

Another way of formulating (\ref{eq:activep}) is by introducing two binary variables $x^{P^+}_{c,g},\, x^{P^-}_{c,g} \in \{0,1\}$ for every $c\in\mathcal{C}$ and $g\in\mathcal{G}$,  to indicate the mode of operation. Then, the three conditions in (\ref{eq:activep}) can be stated as
\begin{subequations}\label{eq:mixa1}
%{\small{
\begin{align}
&\!\!\!p^{\mathrm{gen}}_{0,g}\!+\!\alpha_{c,g}\Delta_c \!-\! p^{\mathrm{gen}}_{c,g} \leq M_{c,g}(1\!-\!x^{P^+}_{c,g})\; &&\hspace{0mm}\forall c\in\mathcal{C}, \; g\in\mathcal{G},\!\! \label{eq:mixa11}\\
&\!\!\!p^{\mathrm{gen}}_{c,g}\!-\!p^{\mathrm{gen}}_{0,g}\!-\!\alpha_{c,g}\Delta_c \leq M_{c,g}(1\!-\!x^{P^-}_{c,g})\; &&\hspace{0mm}\forall c\in\mathcal{C}, \; g\in\mathcal{G},\!\! \label{eq:mixa12}\\
&\!\!\!p^{\mathrm{max}}_{c,g}-p^{\mathrm{gen}}_{c,g} \leq (p^{\mathrm{max}}_{c,g}-p^{\mathrm{min}}_{c,g})\,x^{P^+}_{c,g}\; &&\hspace{0mm}\forall c\in\mathcal{C}, \; g\in\mathcal{G},\!\! \label{eq:mixa13}\\
&\!\!\!p^{\mathrm{gen}}_{c,g}-p^{\mathrm{min}}_{c,g} \leq (p^{\mathrm{max}}_{c,g}-p^{\mathrm{min}}_{c,g})\,x^{P^-}_{c,g}\; &&\hspace{0mm}\forall c\in\mathcal{C}, \; g\in\mathcal{G},\!\! \label{eq:mixa14}
\end{align}%}}
\end{subequations}
where the ``big-M'' multipliers, $M_{c,g}$, are chosen sufficiently large to ensure that (\ref{eq:mixa1}) is equivalent to (\ref{eq:activep}).
Observe that according to (\ref{eq:mixa11}) and (\ref{eq:mixa12})
\begin{align}
&x^{P^+}_{c,g} = x^{P^-}_{c,g}=1 \;\;\Rightarrow\;\; p^{\mathrm{min}}_{c,g}\leq p^{\mathrm{gen}}_{c,g} = p^{\mathrm{gen}}_{0,g}+\alpha_{c,g}\Delta_c\leq p^{\mathrm{max}}_{c,g}\nonumber\\
&x^{P^+}_{c,g}=1,\; x^{P^-}_{c,g}=0 \;\;\Rightarrow\;\; p^{\mathrm{max}}_{c,g}=p^{\mathrm{gen}}_{c,g}\leq p^{\mathrm{gen}}_{0,g}+\alpha_{c,g}\Delta_c\nonumber\\
&x^{P^+}_{c,g}=0,\; x^{P^-}_{c,g}=1 \;\;\Rightarrow\;\; p^{\mathrm{gen}}_{0,g}+\alpha_{c,g}\Delta_c\leq p^{\mathrm{gen}}_{c,g} = p^{\mathrm{min}}_{c,g}\nonumber\\
&x^{P^+}_{c,g} = x^{P^-}_{c,g}=0 \;\;\Rightarrow\;\; p^{\mathrm{min}}_{c,g}= p^{\mathrm{gen}}_{c,g} = p^{\mathrm{max}}_{c,g}.\nonumber
\end{align}

%Equations (\ref{eq:mixa11}) and (\ref{eq:mixa12}), when $x^{P^+}_{c,g} = x^{P^-}_{c,g}=1$, simply amount to (\ref{eq:activep1}) where $p^{\mathrm{gen}}_{c,g} = p^{\mathrm{gen}}_{0,g}+\alpha_{c,g}\Delta_c$. Similarly, (\ref{eq:mixa13}) and (\ref{eq:mixa14}) when $x^{P^+}_{c,g} = x^{P^-}_{c,g}=0$ amount to (\ref{eq:activep2}) and (\ref{eq:activep3}), respectively, by forcing $p^{\mathrm{gen}}_{c,g}$ to be equal to $p^{\mathrm{max}}_{c,g}$ and $p^{\mathrm{min}}_{c,g}$.

Additionally, 
generator active power contingency response can be expressed using Min and Max operators as
 %{\small{ 
\begin{align}
\!\!\!\pbf^{\mathrm{gen}}_c\!=\!\max\{\pbf_c^{\min}\!,\min\{\Cbf_{\!c}(\pbf^{\mathrm{gen}}_0\!+\!\boldsymbol{\alpha}_c\Delta_c),\pbf^{\max}_c\}\} \;\;\; \forall c\!\in\!\mathcal{C},\!\!\! \label{eq:minmaxa}
\end{align}%}}
which can be equivalently formulated based on the defined set~(\ref{eq:set_orig}), for every $c \in \Ccal$ and $g \in \Gcal$, as
{\small
\begin{align} 
\!\!\!\!\Big(\frac{
	2p^{\mathrm{gen}}_{c,g}-\!p^{\max}_{c,g}\!+\!p^{\min}_{c,g}
}{
	p^{\max}_{c,g}+p^{\min}_{c,g}},\frac{2(p^{\mathrm{gen}}_{0,g}\!+\!\alpha_{c,g}\Delta_c)\!-p^{\max}_{c,g}\!+\!p^{\min}_{c,g}} {p^{\max}_{c,g}+p^{\min}_{c,g}
}\Big)
\!\in\! \Fcal_{\frac{\pi}{4}}.\!\!\!\! \label{eq:minmaxa1}
\end{align}}
\noindent \!\!\!\! Equations (\ref{eq:activep}) - (\ref{eq:minmaxa1}) are all equivalent and imply a piecewise-smooth model as shown in Figure~\ref{fig:fig1} (a).

 \begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{figures/ongp1.pdf}
	\caption{Generator active power response relation between pre- and post-contingency: (a) Actual characteristics: $x=p^{\mathrm{gen}}_{c,g}$, $y=p^{\mathrm{gen}}_{0,g}+\alpha_{c,g}\Delta_c$, (b) Normalization of the actual characteristics: $\hat{x}=\frac{2p^{\mathrm{gen}}_{c,g}-p^{\max}_{c,g}+p^{\min}_{c,g}}{p^{\max}_{c,g}+p^{\min}_{c,g}}$, $\hat{y}=\frac{2(p^{\mathrm{gen}}_{0,g}+\alpha_{c,g}\Delta_c)-p^{\max}_{c,g}+p^{\min}_{c,g}} {p^{\max}_{c,g}+p^{\min}_{c,g}}$.}
	\label{fig:fig1}
\end{figure}
 \subsection{Generator Reactive Power Contingency Response}
Ideally, the generators that contribute to a given contingency redispatch may need to readjust their post-contingency reactive power production in order to retain the base case voltage magnitude,
\begin{align}
|v_c|=|v_0|.
\end{align}
However, in the presence of tight reactive power limits, maintaining pre-contingency voltage magnitudes might not be possible. Therein, 
\begin{itemize}
\item the bus voltage magnitude can drop below its base-case level if all generator reactive power upper limits of the bus are binding;
\item  the bus voltage magnitude is allowed to rise above its base-case level if all generator reactive power lower limits of the bus are binding.
\end{itemize}
%then the generator must operate to provide maximum reactive power. Similarly, if the bus voltage magnitude becomes greater than the base-case level, the generator is supposed to provide minimum reactive power. 
This requirement can be formulated as follows: 
%{\small{
\begin{subequations}\label{eq:ractivep}
\begin{align}
&\!\!\! q^{\min}_{c,g} \!\leq\! q^{\mathrm{gen}}_{c,g} \!\leq\! q^{\max}_{c,g} ,&&\hspace{-1mm}|v_{c,i}|\!=\!|v_{0,i}|&&&&\hspace{-4mm} \forall c \!\in\! \Ccal, g \!\in\! \Gcal, i \!\in\! \Ncal,\!\!\!\! \label{eq:ractivep1}\\
&\!\!\! q^{\mathrm{gen}}_{c,g} = q^{\max}_{c,g} ,&&\hspace{-1mm}|v_{c,i}|\!<\!|v_{0,i}|&&&&\hspace{-4mm} \forall c \!\in\! \Ccal, g \!\in\! \Gcal, i \!\in\! \Ncal,\!\!\!\! \label{eq:ractivep2} \\
&\!\!\! q^{\mathrm{gen}}_{c,g} = q^{\min}_{c,g} ,&&\hspace{-1mm}|v_{c,i}|\!>\!|v_{0,i}|&&&&\hspace{-4mm} \forall c \!\in\! \Ccal, g \!\in\! \Gcal, i \!\in\! \Ncal.\!\!\!\!\label{eq:ractivep3}
\end{align}
\end{subequations}%}}

Alternatively, we can reformulate (\ref{eq:ractivep}) with respect to auxiliary binary variables: %Min and Max operators;
\begin{subequations}\label{eq:mixr1}
	%{\small{
\begin{align}
&|v_{0,i}|\!-\!|v_{c,i}| \leq (v^{\mathrm{max}}_{i}\!-\!v^{\mathrm{min}}_{i})(1\!-\!x^{Q^+}_{c,g}) 
&&\hspace{0mm}\forall c\!\in\!\mathcal{C},  g\!\in\!\mathcal{G},\!\! \label{eq:mixr11}\\
&|v_{c,i}|\!-\!|v_{0,i}| \leq (v^{\mathrm{max}}_{i}\!-\!v^{\mathrm{min}}_{i})(1\!-\!x^{Q^-}_{c,g}) 
&&\hspace{0mm}\forall c\!\in\!\mathcal{C},  g\!\in\!\mathcal{G},\!\! \label{eq:mixr12}\\
&q^{\mathrm{max}}_{c,g}\!-\!q^{\mathrm{gen}}_{c,g} \leq (q^{\mathrm{max}}_{c,g}\!-\!q^{\mathrm{min}}_{c,g})x^{Q^+}_{c,g}\!\!\!\! &&\hspace{0mm}\forall c\!\in\!\mathcal{C}, \, g\!\in\!\mathcal{G},\!\! \label{eq:mixr13}\\
&q^{\mathrm{gen}}_{c,g}\!-\!q^{\mathrm{min}}_{c,g} \leq (q^{\mathrm{max}}_{c,g}\!-\!q^{\mathrm{min}}_{c,g})x^{Q^-}_{c,g}\!\!\!\! &&\hspace{0mm}\forall c\!\in\!\mathcal{C}, \, g\!\in\!\mathcal{G}.\!\! \label{eq:mixr14}
\end{align}%}}
\end{subequations}
where $i\in\mathcal{N}$ is the bus where $g$ is located and $x^{Q^+}_{c,g},\, x^{Q^-}_{c,g} \in \{0,1\}$ denote the introduced binary variables. Observe that
\begin{align}
&x^{Q^+}_{c,g}= x^{Q^-}_{c,g} = 1 \;\Rightarrow\;|v_{c,i}|=|v_{0,i}|\;\wedge\;
q^{\mathrm{min}}_{c,g}\leq q^{\mathrm{gen}}_{c,g}\leq q^{\mathrm{max}}_{c,g},\nonumber\\
&x^{Q^+}_{c,g}=0,\;\; x^{Q^-}_{c,g} = 1 \;\Rightarrow\;|v_{c,i}|\leq|v_{0,i}|\;\wedge\;
q^{\mathrm{gen}}_{c,g}= q^{\mathrm{max}}_{c,g},\nonumber\\
&x^{Q^+}_{c,g}=1,\;\; x^{Q^-}_{c,g} = 0 \;\Rightarrow\;|v_{c,i}|\geq|v_{0,i}|\;\wedge\;
q^{\mathrm{gen}}_{c,g}= q^{\mathrm{min}}_{c,g},\nonumber\\
&x^{Q^+}_{c,g}= x^{Q^-}_{c,g} = 0 \;\Rightarrow\;
q^{\mathrm{min}}_{c,g}= q^{\mathrm{gen}}_{c,g}= q^{\mathrm{max}}_{c,g}.\nonumber
\end{align}

%Equations (\ref{eq:mixr11}) and (\ref{eq:mixr12}), when $x^{Q^+}_{c,g} = x^{Q^-}_{c,g}=1$, ensure equality, $|v_{c,i}|=|v_{0,i}|$, as represented in (\ref{eq:ractivep1}). Similarly, (\ref{eq:mixr13}) and (\ref{eq:mixr14}), when $x^{Q^+}_{c,g} = x^{Q^-}_{c,g}=0$, respectively, ensure $q^{\mathrm{gen}}_{c,g}$ to be equal to $q^{\mathrm{max}}_{c,g}$ and $q^{\mathrm{min}}_{c,g}$.

In addition to the representation in (\ref{eq:ractivep}) and (\ref{eq:mixr1}), for every $c\in\Ccal$,
generator reactive power contingency response can be expressed using Min and Max operators as follows:
%{\small{
\begin{align}
 &\!\!\!\!\!\!\min\!\big\{\!\max\{0,\Gbf_c(|\vbf_0|\!-\!|\vbf_c|)\},\max\{0,\qbf^{\max}_c\!-\!\qbf^{\mathrm{gen}}_c\}\big\}\!=\!\nonumber\\
&\!\!\!\!\!\!\min\!\big\{\!\max\{0,\Gbf_c(|\vbf_c|\!-\!|\vbf_0|)\},\max\{0,\qbf^{\mathrm{gen}}_c\!-\!\qbf^{\min}_c\}\big\}\!=\!0. \!\!\!\!
\end{align}%}}
%\noindent 
Equation (\ref{eq:ractivep})  can be equivalently formulated based on the defined set (\ref{eq:set_orig}) for every $c \in \Ccal$, $g \in \Gcal$ and $i \in \Ncal$ as
%{\small 
\begin{align} 
\Big(\frac{2q^{\mathrm{gen}}_{c,g}-q^{\max}_{c,g}-q^{\min}_{c,g}}
{q^{\max}_{c,g}-q^{\min}_{c,g}},\;\; |v_{0,i}|-|v_{c,i}|\Big) \in \Fcal_{0}.\label{eq:minmaxr1}
\end{align}%}

The formulations, (\ref{eq:ractivep}) -- (\ref{eq:minmaxr1}), refer to the PV/PQ switching as demonstrated in Figure~\ref{fig:fig2} (a). Herein, PV bus means that the bus voltage magnitude and the generation level of active power are fixed whereas its voltage phase angle and reactive power generation are varying. When it hits the reactive power capacity limits to sustain the value of voltage magnitude in the base case, the bus type needs to become PQ. This bus type means that the power generations, e.g., real and reactive, are constant, whereas the voltage magnitude and phase angle are varying. Similar to the characteristic of active power, reactive power contingency response implies a piecewise-smooth  model. %where its solution space is not only highly nonlinear, but also disconnected. 

\begin{figure}[h]
	\centering 
	\includegraphics[width=\columnwidth]{figures/ongq11.pdf}
	\caption{Generator reactive power response relation between pre- and post-contingency: (a) Actual characteristics: $x=q^{\mathrm{gen}}_{c,g}$, $y=|v_{0,i}|-|v_{c,i}| $, (b) Normalization of the actual characteristics: $\hat{x}=\frac{2q^{\mathrm{gen}}_{c,g}-q^{\max}_{c,g}-q^{\min}_{c,g}}{q^{\max}_{c,g}-q^{\min}_{c,g}}$, $\hat{y}=|v_{0,i}|-|v_{c,i}|$.}
	\label{fig:fig2}
\end{figure} 

\section{Security-constrained Optimal Power Flow}

This section elaborates the active and reactive power contingency response models. Herein, devised objective function minimizes the generational cost in the base case and secures the grid to contingency scenarios.% A general formulation is given as %\begin{subequations}\label{eq:gen}
%	\begin{align}
%	&\hspace{-2.0mm} \underset{
%				\begin{subarray}{c} 
%				\ubf_c,\xbf_c \forall c \in {\{0\} \cup \mathcal{C}}
%				\end{subarray}
%	}{\text{minimize~~~}}
%	&&\hspace{-0.0cm}  f(\xbf_0, \ubf_0) 
%	\hspace{-5mm}   \hspace{0mm}\label{eq:gen_obj}\\ \nonumber \\
%	&\hspace{-1.0mm} \text{subject to~~~~~~~}
%	&&\hspace{-0.0cm} \gbf_c(\xbf_c, \ubf_c)=\bm{0} &&&& \hspace{1.25cm}\forall c\in\mathcal{C},\hspace{0mm} \label{eq:gen1}\hspace{0mm}\\
%	&\hspace{-0.0mm}&&\hspace{-0.0cm}\hbf_c(\xbf_c, \ubf_c) \leq \bm{0} &&&& \hspace{1.25cm}\forall c\in\mathcal{C},\hspace{0mm} \label{eq:gen2}\\
%	&\hspace{-0.0mm}&&\hspace{-0.0cm}|\ubf_c-\ubf_0| \;\,\leq \bar{\ubf}_c^{\max} &&&& \hspace{1.25cm}\forall c\in\mathcal{C}.\hspace{0mm} \label{eq:gen3}
%	\end{align}
%	%	\vspace{-6.5mm}
%\end{subequations}
%where $\xbf_0$ and $\xbf_c$ represent the state variables, such as nodal voltage magnitude for base and contingency case, respectively.  $\ubf_0$ and $\ubf_c$ represents the decision variables, such as generator power production for base and contingency case, respectively. Equation (\ref{eq:gen1}) represents the physical constraints, such as nodal power balance, while inequality (\ref{eq:gen2}) denotes the operational constraints, such as generator capacity limits. The constraints (\ref{eq:gen3}) imposes the maximum permissible variation in decision variables between pre- and post-contingency case.\\

\subsection{Non-differentiable Contingency Response in SCOPF Formulation}

SCOPF with respect to the outage of an arbitrary set of generators and lines can be formulated as 
{\small{
\begin{subequations}\label{eq:OPFLC}
%	\vspace{-4.5mm}
	\begin{align}
	&\hspace{-0.0mm} \underset{
		%		\begin{subarray}{c} 
		%		\pbf^{\mathrm{gen}}_c,\qbf^{\mathrm{gen}}_c\in\mathbb{R}^{|\mathcal{G}|}\\
		%		\pbf^{\mathrm{imb}}_c,\qbf^{\mathrm{imb}}_c\in\mathbb{R}^{|\mathcal{N}|}\\
		%		\vec{\pbf}_c,\cev{\pbf}_c,\vec{\qbf}_c,\cev{\qbf}_c,\sbf^{\mathrm{vio}}_c\in\mathbb{R}^{|\mathcal{L}|}\\
		%		\Wbf_c\in\mathbb{H}_{|\mathcal{N}|},
		%		\vbf_c\in\mathbb{C}^{|\mathcal{N}|}\\
		%		\Delta_c\in\mathbb{R}
		%		\end{subarray}
	}{\text{~~~minimize~~~}}
	&&\hspace{-0.5cm}  h(\pbf^{\mathrm{gen}}_0) 
	\hspace{-5mm}   \hspace{0mm}\label{eq:OPFLC_obj}\\ \nonumber \\
	&\hspace{-0.0mm} \text{~~~subject to~~~~~~~} && &&&&\nonumber\\
	&&&\hspace{-2.25cm}\sbf^{\mathrm{dem}}_c+\mathrm{diag}\{\!\vbf_c\vbf_c^{\ast}\,\Ybf^{\ast}_{\!c}\} 
	=\Gbf^{\top}_c(\pbf^{\mathrm{gen}}_c+i \qbf^{\mathrm{gen}}_c) &&&& \hspace{-2.5cm}\forall c\in\mathcal{C}\hspace{0mm} \label{eq:OPFLC_cons_4}\hspace{0mm}\\
	&\hspace{-0.0mm}&&\hspace{-2.25cm}|\mathrm{diag}\{\vec{\Lbf}_c^{\phantom{\ast}}\;\!\vbf_c\vbf_c^{\ast}\,\vec{\Ybf}^{\ast}_{\!c}\}|\leq\sbf^{\mathrm{max}}_c &&&& \hspace{-2.5cm}\forall c\in\mathcal{C}\hspace{0mm} \label{eq:OPFLC_cons_5}\\
	&\hspace{-0.0mm}&&\hspace{-2.25cm}|\mathrm{diag}\{\cev{\Lbf}_c^{\phantom{\ast}}\;\!\vbf_c\vbf_c^{\ast}\,\cev{\Ybf}^{\ast}_{\!c}\}|\leq\sbf^{\mathrm{max}}_c &&&& \hspace{-2.5cm}\forall c\in\mathcal{C}\hspace{0mm} \label{eq:OPFLC_cons_6}\\
	&\hspace{-0.0mm}&&\hspace{-2.25cm}\pbf^{\min}_c\leq \pbf^{\mathrm{gen}}_c \leq \pbf^{\max}_c &&&& \hspace{-2.5cm}\forall c\in\mathcal{C}\hspace{0mm}  \label{eq:OPFLC_cons_7}\\
	&\hspace{-0.0mm}&&\hspace{-2.25cm}\qbf^{\min}_c\leq \qbf^{\mathrm{gen}}_c \leq \qbf^{\max}_c &&&& \hspace{-2.5cm}\forall c\in\mathcal{C}\hspace{0mm}  \label{eq:OPFLC_cons_8}\\
	&\hspace{-3.0mm}&&\hspace{-2.25cm}\vbf^{\min}\leq|\vbf_c|\,\leq\vbf^{\max} &&&& \hspace{-2.5cm}\forall c\in\mathcal{C}\hspace{0mm}  \label{eq:OPFLC_cons_9}\\
	&\hspace{-0.0mm}&& &&&&\nonumber\\
	&\hspace{-0.0mm}&&\hspace{-2.3cm} \Big(\frac{2\pbf^{\mathrm{gen}}_c\!-\!\pbf^{\max}_c\!+\!\pbf^{\min}_c}{\pbf^{\max}_c\!+\!\pbf^{\min}_c},\frac{2\Cbf_{\!c}(\pbf^{\mathrm{gen}}_0\!+\!\boldsymbol{\alpha_c}\Delta_c)\!-\!\pbf^{\max}_c\!+\!\pbf^{\min}_c}
	{\pbf^{\max}_c+\pbf^{\min}_c}\Big) 
	\nonumber\\
	&\hspace{-0.0mm}&&\hspace{-2.3cm} &&&& \hspace{-3.6cm} 
	\in \Fcal_{\frac{\pi}{4}}\,\, \; \forall c\in\mathcal{C}\hspace{0mm} \label{eq:OPFLC_cons_10}\\
	&\hspace{-0.0mm}&&\hspace{-2.3cm}
\Big(\frac{2\qbf^{\mathrm{gen}}_c\!-\!\qbf^{\max}_c\!-\!\qbf^{\min}_c}
{\qbf^{\max}_c-\qbf^{\min}_c}, \Gbf_c(|\vbf_0|\!-\!|\vbf_c|)\Big) \in \Fcal_{0} &&&& \hspace{-2.5cm}\forall c\in\mathcal{C}\hspace{0mm} \label{eq:OPFLC_cons_11}\\
	\nonumber\\
	&\hspace{-0mm}\text{~~~variables}\hspace{-2.0cm} && \hspace{-1cm}  \pbf^{\mathrm{gen}}_0,\pbf^{\mathrm{gen}}_c,\qbf^{\mathrm{gen}}_c, \boldsymbol{\alpha_c} \in\mathbb{R}^{|\mathcal{G}|}; \;  \vbf_0, \vbf_c\in\mathbb{C}^{|\mathcal{N}|}; \; \Delta_c\in\mathbb{R} \nonumber
	\end{align}
\end{subequations}}}
\!\!\!where (\ref{eq:OPFLC_obj}) represents the cost of producing power in the base case. (\ref{eq:OPFLC_cons_4}) fulfills the apparent power balances in the network, whereas  (\ref{eq:OPFLC_cons_5})–(\ref{eq:OPFLC_cons_6}) 
enforce the apparent power flow limits over transmission lines. (\ref{eq:OPFLC_cons_7})–(\ref{eq:OPFLC_cons_8}) represent the generation boundaries for active and reactive power. The inequality (\ref{eq:OPFLC_cons_9}) limits the nodal voltage magnitude. Equation (\ref{eq:OPFLC_cons_10}) represents coupling constraints on generators that relate pre- and post-contingency active power dispatch, while (\ref{eq:OPFLC_cons_11}) stands for the coupling constraints that relate pre- and post-contingency reactive power dispatch with respect to generator capacity limits. It should be noted that  (\ref{eq:OPFLC_cons_10}) and (\ref{eq:OPFLC_cons_11}) are the normalized versions of (\ref{eq:activep}) and (\ref{eq:ractivep}), respectively. 

Constraints (\ref{eq:OPFLC_cons_10}) and (\ref{eq:OPFLC_cons_11}) are major sources of complexity which is due to non-smoothness of the curves $\Fcal_{0}$ and $\Fcal_{\frac{\pi}{4}}$. The main reason behind their normalizations is to conveniently substitute these curves with a smooth sigmoid surrogate. %that transform values on ($-\infty$, $\infty$) into numbers (-1,1) so that (\ref{eq:OPFLC_cons_10}) and (\ref{eq:OPFLC_cons_11}) can be represented in a differentiable model. 
%Accordingly, inverse sigmoid functions transfer values on (-1, 1) into numbers on ($-\infty$, $\infty$). Figures~\ref{fig:fig1}(b) and \ref{fig:fig2}(b) visualize these normalizations. 
In the remainder of this section, we employ different families of continuously-differentiable models as alternatives for (\ref{eq:OPFLC_cons_10}) and (\ref{eq:OPFLC_cons_11}).
 
\subsection{Continuously-differentiable Contingency Response}

The set defined in (\ref{eq:set_orig}) represents a non-differentiable curve. To facilitate the task of local search algorithms, we define a family of continuously-differentiable curves that closely resemble generator contingency responses. 
%To this end, the piecewise-nonsmooth curves, (\ref{eq:OPFLC_cons_10}) and (\ref{eq:OPFLC_cons_11}), can be approximated with continuously-differentiable curves whose coordinates satisfy the smoothed set $\Fcal^{\mathrm{smooth}}_{\theta}$ as 
Such surrogates can be constructed using any of the following sigmoid functions:
\begin{subequations}	\label{eq:14}
	\begin{align}
	&a_1(x)\triangleq\frac{\log(1+x)-\log(1-x)}{2} \label{eq:ac1}\\
	&a_2(x)\triangleq\frac{2}{\pi}\tan\left(\frac{\pi x}{2}\right)\label{eq:ac2}\\
	&a_3(x)\triangleq\frac{x}{\sqrt{1-x^2}}\label{eq:ac3}\\
	&a_4(x)\triangleq\frac{2}{\sqrt{\pi}}\mathrm{ierf}(x)\label{eq:ac4}\\
	&a_5(x)\triangleq\frac{x}{1-|x|}\label{eq:ac5}
	\end{align}
\end{subequations}
that are commonly-used in other areas.  These sigmoids are illustrated in Figure \ref{fig:fig5_1}.

 \begin{figure}[t]
	\centering
	\includegraphics[scale=0.6]{figures/sigmoid.pdf}
	\caption{Sigmoid functions given in (\ref{eq:ac1})-(\ref{eq:ac5}) are normalized at the origin.}
	\label{fig:fig5_1}
\end{figure}


\begin{definition}
Assume that $a:\Rbb\to(-1,1)$ is an arbitrary odd, continuously differentiable, and monotonically increasing function that satisfies
\begin{align}
\lim_{x\to1} a(x)=\infty.
\end{align}
Let $\theta\in[0,\frac{\pi}{2})$, $h>0$, and $k$ be a non-negative integer. Define the family of curves %$\Fcal^{\mathrm{smooth}}_{\theta,\, a,\,h,\,k}$ to be
\begin{align} 
\!\!\!\Fcal^{\mathrm{smooth}}_{\theta,\, a,\,h,\,k}
\triangleq\big\{\big(\frac{a(y)-y}{h}y^{2k}\!+\!\tan(\theta)y,\, y\big)\!\in\!\mathbb{R}^2\;|\;y\!\in\!\Rbb\big\},\!\!\!
\end{align}
as continuously-differentiable surrogates for $\Fcal_{\theta}$.
%\begin{align}
%$f_{\theta,\, a,\,h,\,k}(x)\triangleq h^{-1}(a(x)-x)x^{2k}+\tan(\theta)\,x$. %\label{eq:activation}
%\end{align}
\end{definition}
Constants $h$ and $k$ offer a trade-off between the resemblance with $\Fcal_{\theta}$ and smoothness. This is demonstrated by Figures \ref{fig:fig5}, \ref{fig:fig6}, \ref{fig:fig7} and \ref{fig:fig8}. Constants $\theta$ and $k$ denote the angle of curve and the approximation order at the origin. Figures \ref{fig:fig9} and \ref{fig:fig10} illustrate the resemblance between generator's actual contingency response and candidate curve that are obtained using (\ref{eq:14}).  

Given an appropriate sigmoid and tuning parameters, one can substitute constraints (\ref{eq:OPFLC_cons_10}) and (\ref{eq:OPFLC_cons_11}) with the followings:
\begin{subequations}
{\small
	\begin{align} 
	&\!\Big(\frac{2p^{\mathrm{gen}}_{c,g}\!-\!p^{\max}_{c,g}\!+\!p^{\min}_{c,g}}{p^{\max}_{c,g}+p^{\min}_{c,g}},\frac{2(p^{\mathrm{gen}}_{0,g}\!+\!\alpha_{c,g}\Delta_c)\!-\!p^{\max}_{c,g}\!+\!p^{\min}_{c,g}} {p^{\max}_{c,g}+p^{\min}_{c,g}}\Big)
	%& \nonumber \\
	\!\!\in\! \Fcal^{\mathrm{smooth}}_{\!\frac{\pi}{2},a,h,k}  \\
	&\!\Big(\frac{2q^{\mathrm{gen}}_{c,g}-q^{\max}_{c,g}-q^{\min}_{c,g}}
	{q^{\max}_{c,g}-q^{\min}_{c,g}}, |v_{0,i}|-|v_{c,i}|\Big) \in \Fcal^{\mathrm{smooth}}_{0,\, a,\,h,\,k}.
	\end{align}}
\end{subequations}

%Equation (\ref{eq:activation}) introduces an activation function to integrate approximated curves instead of piecewise-nonsmooth curves. 
%\begin{align}
%f_{\theta}(x)=h^{-1}(a(x)-x)x^{2k}+\tan(\theta)\,x, %\label{eq:activation}
%\end{align}
%where $h$ denotes a smoothing factor that regulates the closeness of a candidate curve to the actual function, while $\theta$ is the angle of curve at the origin. $k$ denotes the order of approximation. The effects of different $h$ values, while $\theta=\pi/4$ and $\theta=0$, on (\ref{eq:ac1})-(\ref{eq:ac5}) are shown in Figures~\ref{fig:fig5} and \ref{fig:fig6}, respectively.
%This function, (\ref{eq:activation}), approximates discrete characteristic of a nerve cell operation by a continuous function. The candidate curve, $a(x)$, chosen among (\ref{eq:ac1}) and (\ref{eq:ac5}) replaces piecewise-nonsmooth curves,  (\ref{eq:OPFLC_cons_10}) and (\ref{eq:OPFLC_cons_11}), with continuously-differentiable functions.


The candidate curves given in (\ref{eq:14}) include inverse hyperbolic tangent (\ref{eq:ac1}), inverse arctangent (\ref{eq:ac2}), inverse algebraic (\ref{eq:ac3}), inverse error (\ref{eq:ac4}), and inverse absolute-value functions. In the following section, we examine the merits of the proposed surrogate functions on the performance of local search algorithms for SCOPF.

\begin{figure*} 
	\centering
	\subfloat(a){%
		\includegraphics[width=0.17\linewidth]{figures/fig5_1.pdf}}
	\hfill
	\subfloat(b){%
		\includegraphics[width=0.17\linewidth]{figures/fig5_2.pdf}}
	\hfill
	\subfloat(c){%
	\includegraphics[width=0.17\linewidth]{figures/fig5_3.pdf}}
	\hfill
	\subfloat(d){%
	\includegraphics[width=0.17\linewidth]{figures/fig5_4.pdf}}
	\hfill
	\subfloat(e){%
	\includegraphics[width=0.17\linewidth]{figures/fig5_5.pdf}}
	\caption{The characteristics of $(x,y) \in \Fcal^{\mathrm{smooth}}_{\pi/4}$ for different $h$ values with the candidate curves: (a) (\ref{eq:ac1}), (b) (\ref{eq:ac2}), (c) (\ref{eq:ac3}), (d) (\ref{eq:ac4}), (e) (\ref{eq:ac5}).}
	\label{fig:fig5} 
\end{figure*}
\begin{figure*} 
	\centering
	\subfloat(a){%
		\includegraphics[width=0.17\linewidth]{figures/fig6_1.pdf}}
	\hfill
	\subfloat(b){%
		\includegraphics[width=0.17\linewidth]{figures/fig6_2.pdf}}
	\hfill
	\subfloat(c){%
		\includegraphics[width=0.17\linewidth]{figures/fig6_3.pdf}}
	\hfill
	\subfloat(d){%
		\includegraphics[width=0.17\linewidth]{figures/fig6_4.pdf}}
	\hfill
	\subfloat(e){%
		\includegraphics[width=0.17\linewidth]{figures/fig6_5.pdf}}
	\caption{The characteristics of $(x,y) \in \Fcal^{\mathrm{smooth}}_{0}$ for different $h$ values with the candidate curves: (a) (\ref{eq:ac1}), (b) (\ref{eq:ac2}), (c) (\ref{eq:ac3}), (d) (\ref{eq:ac4}), (e) (\ref{eq:ac5}).}
	\label{fig:fig6} 
\end{figure*}


\begin{figure*} 
	\centering
	\subfloat(a){%
		\includegraphics[width=0.17\linewidth]{figures/11.pdf}}
	\hfill
	\subfloat(b){%
		\includegraphics[width=0.17\linewidth]{figures/12.pdf}}
	\hfill
	\subfloat(c){%
		\includegraphics[width=0.17\linewidth]{figures/13.pdf}}
	\hfill
	\subfloat(d){%
		\includegraphics[width=0.17\linewidth]{figures/14.pdf}}
	\hfill
	\subfloat(e){%
		\includegraphics[width=0.17\linewidth]{figures/15.pdf}}
	\caption{The characteristics of $(x,y) \in \Fcal^{\mathrm{smooth}}_{\pi/4}$ for different $k$ values with the candidate curves: (a) (\ref{eq:ac1}), (b) (\ref{eq:ac2}), (c) (\ref{eq:ac3}), (d) (\ref{eq:ac4}), (e) (\ref{eq:ac5}).}
	\label{fig:fig7} 
\end{figure*}
\begin{figure*} 
	\centering
	\subfloat(a){%
		\includegraphics[width=0.17\linewidth]{figures/21.pdf}}
	\hfill
	\subfloat(b){%
		\includegraphics[width=0.17\linewidth]{figures/22.pdf}}
	\hfill
	\subfloat(c){%
		\includegraphics[width=0.17\linewidth]{figures/23.pdf}}
	\hfill
	\subfloat(d){%
		\includegraphics[width=0.17\linewidth]{figures/24.pdf}}
	\hfill
	\subfloat(e){%
		\includegraphics[width=0.17\linewidth]{figures/25.pdf}}
	\caption{The characteristics of $(x,y) \in \Fcal^{\mathrm{smooth}}_{0}$ for different $k$ values with the candidate curves: (a) (\ref{eq:ac1}), (b) (\ref{eq:ac2}), (c) (\ref{eq:ac3}), (d) (\ref{eq:ac4}), (e) (\ref{eq:ac5}).}
	\label{fig:fig8} 
\end{figure*}


\begin{figure*} 
	\centering
	\subfloat(a){%
		\includegraphics[width=0.17\linewidth]{figures/t1.pdf}}
	\hfill
	\subfloat(b){%
		\includegraphics[width=0.17\linewidth]{figures/t2.pdf}}
	\hfill
	\subfloat(c){%
		\includegraphics[width=0.17\linewidth]{figures/t3.pdf}}
	\hfill
	\subfloat(d){%
		\includegraphics[width=0.17\linewidth]{figures/t4.pdf}}
	\hfill
	\subfloat(e){%
		\includegraphics[width=0.17\linewidth]{figures/t5.pdf}}
	\caption{The characteristics of $(x,y) \in \Fcal^{\mathrm{smooth}}_{\pi/4}$ for the $k$ and $h$ values used in simulations with the candidate curves: (a) (\ref{eq:ac1}), (b) (\ref{eq:ac2}), (c) (\ref{eq:ac3}), (d) (\ref{eq:ac4}), (e) (\ref{eq:ac5}).}
	\label{fig:fig9} 
\end{figure*}
\begin{figure*} 
	\centering
	\subfloat(a){%
		\includegraphics[width=0.17\linewidth]{figures/t1_1.pdf}}
	\hfill
	\subfloat(b){%
		\includegraphics[width=0.17\linewidth]{figures/t2_2.pdf}}
	\hfill
	\subfloat(c){%
		\includegraphics[width=0.17\linewidth]{figures/t3_3.pdf}}
	\hfill
	\subfloat(d){%
		\includegraphics[width=0.17\linewidth]{figures/t4_4.pdf}}
	\hfill
	\subfloat(e){%
		\includegraphics[width=0.17\linewidth]{figures/t5_5.pdf}}
	\caption{The characteristics of $(x,y) \in \Fcal^{\mathrm{smooth}}_{0}$ for the $k$ and $h$ values used in simulations with the candidate curves: (a) (\ref{eq:ac1}), (b) (\ref{eq:ac2}), (c) (\ref{eq:ac3}), (d) (\ref{eq:ac4}), (e) (\ref{eq:ac5}).}
	\label{fig:fig10} 
\end{figure*}
 


==> PV_PQ paper/intro.tex <==


\section{Introduction}
\seclabel{intro}
% 
%\IEEEPARstart{E}{ver} increasing penetration of distributed generation (DG) unit in distribution network has triggered the concept of optimal operation of DGs. The introduction of DG, by which the distribution networks are changed into a source owned system, may cause lots of variation on the characteristics of the power flow \cite{pf_dgs}. 

\IEEEPARstart{P}{ower} flow analysis underpins many static and dynamic applications, including stability analysis, optimal power flow, contingency analysis, etc. Accurate power flow solutions ensure the generation-demand balance under all circumstances. However, since transmission losses cannot be identified a priori, the total power needed to supply a known demand remains unpredictable \cite{investigate_dsb}. The common practice is to assume that there exist at least one slack bus, where active power generation can be readjusted to compensate for imbalances\cite{book1, l3}. Power flow models that are based on multiple slack buses alleviate the burden of a pre-specified single slack bus by dispatching the imbalance among participating sources  \cite{incre_ping}. This approach better mimics the operation of power systems provided that participation factors of generators are accurately determined. These participation factors can be appointed based on machine inertia \cite{unbund_ilic}, governor droop characteristics \cite{droop1,virtual}, frequency control \cite{slack_sel}, and economic dispatch \cite{ecd_part,incre_meisel, jang2005modified}. Another major aspect of post-contingency analysis is the determination of reactive power dispatch and voltage magnitudes \cite{novelopf}. When the reactive power limit of a generator is reached, it cannot maintain predefined voltage settings, and the bus type should inevitably switch from PV bus to PQ bus \cite{l11}. The active and reactive power limits are handled via controller design \cite{l8}, \cite{upf} by sacrificing the optimal operation. Moreover, possible component outage, i.e. generator or line, are rarely studied in the literature \cite{l7}.

% The use of the resulting converged power flow plus a linear proportional sharing principle \cite{loadloss_strbac2} make it possible for the allocation of losses to generators and consumers. 
%, is paid much less attention for a long term
%The study of possible component outage, i.e. generator or line, however, is rare in the literature \cite{6348,participation_tong} .
 
%Distributed slack bus modeling in response to line and generator outage was studied in \cite{6348}. The network topology and load distribution variations are considered in \cite{participation_tong}.  

%Virtual multi-slack droop control based on power sensitivity analysis is proposed for providing proper load sharing among generators in islanded networks \cite{virtual}. The participation factors that use combined cost and reliability criteria in power flow for fair pricing is proposed in \cite{unbund_ilic}. These studies, however, only focus on having all generators contributing the losses regardless of increased transmission losses. It is shown that distributing the system imbalance among several generators may not lead to lower losses \cite{slack_sel}. To this end, proper selection of slack bus among all available DGs can pave the way for optimal operation of power networks.
%This can be tackled by the extension of the power flow formulation to the SCOPF formulation, which considers contingency constraints.
Security-constrained optimal power flow (SCOPF) formulations focus on the optimization of a robust power dispatch with respect to the outage of arbitrary sets of generators or lines \cite{l2,l3}. 
%Preventive models of SCOPF find operational strategies that are identical, i.e., no redispatch,  in transition from pre- to post-contingency scenarios \cite{l6}. Preventive SCOPF usually ignores generator failures in contingency states \cite{l4}. On the contrary, 
Corrective models of SCOPF allow limited adjustment of operating points in response to contingencies, i.e., redispatch, in post-contingency scenarios \cite{l5}. 
%Corrective SCOPF considers both generator and transmission line contingencies. 
In this case, to account for a realistic post-contingency behavior of generators, additional constraints have to be incorporated into corrective models of SCOPF formulation \cite{l10}. These additional constraints are based on nonsmooth, i.e., discontinuous, curves of real and reactive power responses to avoid prevent both active and reactive power violations \cite{l9}. However, nonsmooth models prevent the use of power flow algorithms due to non-differentiability  \cite{l12}. This problem, and its possible adverse consequences, such as an increased iteration count and convergence to an unstable region, have been discussed in \cite{l9}.

Alternative differentiable power flow models using hyperbolic and sigmoid functions \cite{l10}, patching functions with complementary homotopy methods \cite{l12}, and discrete and continuous auxiliary variables, are discussed in \cite{l11}. %These methods are not validated for an arbitrary set of outages, i.e. a generator or a line, and their performance depends on a specific numerical solver. 
In this paper, we introduce several continuously-differentiable models that respect high-fidelity physical models of generators considering an extensive list of contingency scenarios. These models prevent physical and operational violations by means of optimally allocating active power imbalances among available generators and deciding the bus type, i.e., PV/PQ switching, respectively. While the employed local search solver fail to converge using continuous complementarity condition from \cite{l11}, the proposed model enable the recovery of fully feasible solutions in all of the simulated cases. 
%{\color{red}{is that all? the list of our contribution seems rather short or not sufficiently detailed?}} %The proposed SCOPF formulation is in a generic form, and can be solved with various numerical solvers.


The rest of this paper has the following organization. Section II discusses the preliminary materials. Section III elaborates the enhanced modeling of the generator response including representation of a distributed slack bus as well as active and reactive power contingency response models for a generator. Section IV introduces several continuously-differentiable models that account for active and reactive power contingency responses in the SCOPF formulation. In Section V, the proposed enhanced modeling of generator response in SCOPF solution is verified through a numerical benchmark system. Section VI concludes the paper.






%Power flow equations along with sensitivity analysis are used to allocate active transmission losses among market participants \cite{sensitivity}.
% proves that a single slack bus offer less system loss assuming that no upper limit are imposed on slack powers. In the presence of upper limits, it is concluded that distributed slack bus is needed).


%This has become much more important to be able to determine which generators are supply a particular load, how much use each generator is making of a transmission line and what is each generators contribution to the system losses\cite{app_dsb}.


%Even though many work has been done in distributed slack bus model, competition in the electricity supply industry is limited to a few study \cite{virtual,sensitivity}. 




%The concept of distributed slack bus based power-flow analysis for unbalanced transmission networks \cite{unbalanced} and unbalanced distribution grids \cite{dsb_distgrid} has been addressed in the technical literature. \cite{sensitivity} uses power flow equations along with sensitivity techniques to allocate active transmission losses among market participants. \cite{app_dsb} disperses the power imbalance to voltage controlled buses in the system based on the participation factor obtained by the average of automatic generation control. \cite{upf} extends the \cite{app_dsb} for islanded networks. Virtual multi-slack droop control based on power sensitivity analysis is proposed for providing proper load sharing among generators in islanded microgrids \cite{virtual}.

% The participation factors were incorporated in three-phase power flow equations which were solved using a Newton-Raphson algorithm \cite{unbalanced}.




% When a distributed slack bus is adopted, all active power mismatches are retained in the unknown vector while the state vector gets augmented with the system power imbalance in order to compensate for the missing phase reference \cite{unbund_ilic,ecd_part,incre_ping}. Nonzero elements of the extra Jacobian column are simply the respective participation factors. In addition to the stand-alone load-flow problem, participation factors frequently arise in other applications where the load-flow problem constitutes the core, like economic dispatch \cite{ecd_part,incre_meisel} deregulated markets \cite{incre_ping}.



%\cite{unbund_ilic} applied the distributed slack bus with participation factors which use combined cost and reliability criteria in power flow for fair pricing. it is shown that distributing the system imbalance among several generators may lead to lower losses (\cite{slack_sel} proves that a single slack bus offer less system loss assuming that no upper limit are imposed on slack powers. in the presence of upper limit, it is concluded that distributed slack bus is needed).

%The slack bus issue arises primarly because of lack of prior knowledge of system losses. Because of this, to maintain the real power balance on the system cannot specify the real power generated at all generators. The computed losses on the transmission system are a function of the choice of a slack bus. For example, computations using a slack bus electrically distant from the points of a certain transaction might indicate either infeasibility of the transaction or high losses associated with it. In the actual operation of electric power systems there is no single slack bus. To account for this a distributed slack bus must be used. The pricing for losses or imbalances on the system should correspond to actual operation for the pricing scheme to be fair.


%The slack bus is a mathematical artifact that does not fully reflect actual operation of electric power systems. Instead, there exist a relatively small number of generating units designated as load following units. These units participate in the load frequency  control and automatic generation control with the purpose of balancing the interconnected system in response to demand uncertainties. They effectively manage to maintain system frequency at 60 Hz. These units are distributed at various geographics locations in the system. They are necessary in order to make a transaction feasible without degrading the quality of supply and reliablity of the system. The amount of real power imbalance in the system is distributed among these units based on participation factors. These are determined based on combined cost and reliability criteria.       

%\cite{incre_meisel} provides a method of choosing participation factors based on the minimal incremental change in generation costs.
%This paper presents the participation factor load-flow formulation which includes a participation vector used to distribute the mismatch in real power between the specified total generation and the specified total demand plus system losses.


%The steady-state analysis of bulk electric power systems, commonly known as the load-flow problem, has usually involved the designation of one generator as the slack-bus generator. Numerous authors have suggested that the slack-bus constraints is not really necessary in computer-based load flow formulations \cite{dist_slack1,6348}

%distributed slack bus feature in response to line and generator outage was studied in \cite{6348}.The mismatch of generation, load and metwork loss is distributed among the buses.




%\cite{loadloss_strbac1} distinguishes the load and loss contribution by each generator.


%because of the introduction of competition in the electricity supply industry, it has become much more important to be able to determine which generators are supply a particular load, how much use each generator is making of a transmission line and what is each generators contribution to the system losses.
%The transmission network is a natural monopoly and should remain centrally controlled. it is also widely recognized that the operation of the transmission system can have enormous impact on a competitive market.In this respect, generators, suppliers and network operating companies are likely to want accurate and indisputable answers o questions such as " how far is the power generated by this unit really going?" or "which generators are supplying this load?" or even "which generator is making the biggest use of this transmission line?"



%The use of a distributed slack bus avoids concentrating the cumulative injection error at a single bus\cite{dist_slack1}. 


%The mismatch of generation, load and metwork loss is distributed among the buses within the voltage correction iteration rather than after each iteration.




%Droop control has been attached to distributed generators in order to meet above-given requirements of islanded networks \cite{droop1}. Heuristic optimization (Particle swarm optimization) method incorporated droop control is used to eliminate single slack bus assumption for autonomous microgrids \cite{pso}.  

%A slack bus has two meanings in the conventional power flow analysis. One is the angle reference bus, and the other is the bus which compensates the unbalances resulted from losses. Without the angle reference bus, the Jacobian matrix will certainly be singular.


%Participation factor with a sense of economic load dispatch, in which every generator maintains equal incremental cost, was proposed in \cite{jang2005modified}.


%A distributed slack bus model has been developed in \cite{unbalanced} using the concept of participation factors, applicable to unbalanced systems. The participation factors were incorporated in three-phase power flow equations which were solved using a Newton-Raphson algorithm. Such a model can be used for DG placement studies, network reconfiguration, economic analysis for fair pricing and aggregate substations loading.

%The concept of DSB-based power-flow analysis for balanced transmission networks \cite{unbalanced} and unbalanced distribution grids \cite{dsb_distgrid} has been addressed in the technical literature.


%\cite{sensitivity} uses power flow equations along with sensitivity techniques to allocate active transmission losses among market participants. 

%\cite{app_dsb} disperses the power imbalance to voltage controlled buses in the system based on the participation factor obtained by the average of automatic generation control. \cite{upf} extends this for islanded networks.




%Literature suggests that the power flow for an islanded microgrid cannot be solved using conventional approaches, hence the conventional method like Newton Raphson (which is most widely used in power system studies) cannot be applied to islanded microgrids. Conventional load flow algorithms are valid when slack bus is present and system frequency is constant i.e. grid connected mode. 

%Now, since the system frequency is not constant in an islanded microgrid, the Ybus is also not constant because the reactance in the Ybus depends on the frequency. Also, the conventional assumption to classify the droop bus (the bus at which the DG is connected) either as slack, PV or PQ bus in a power flow is invalid as the active and reactive powers as well as the voltage magnitude and angle of the droop bus are not pre-specified and depend upon the system parameters so conventional methods are not applicable in case of an islanded microgrid \cite{seq_frame}. 




%\cite{loc_mar}
%\cite{evolutionary}
%\cite{marg_loss}
%\cite{iterative} 
%\cite{smart_grid}
%\cite{slack_nr}
%\cite{gen_hybrid}
%
%\cite{stability_mgs}
%\cite{convex_dsb}





%\subsection{literature search}
%
%\cite{l1}, \cite{dist_slack1}, \cite{incre_meisel}, \cite{unbund_ilic}, \cite{incre_ping}, \cite{participation_tong}, \cite{slack_sel}, \cite{jang2005modified}, \cite{unbalanced} $\rightarrow$ these papers handle the mismatch of generation, load and network losses by distributing them among all the generator with participation factor for base case scenario. They don't consider reactive power limits or contingency scenarios. Also, solution approach is Newton-Raphson for all.   
%
%
%
%\cite{seq_frame}, \cite{droop1},\cite{virtual}, \cite{upf} $\rightarrow$ handle active-reactive power limits via droop control design but this is not integrated into problem formulation. (Newton raphson)
%
%\cite{l2}, \cite{l3},\cite{l6} deals with post contingency corrective (preventive) control action using battery energy storage or FACTS devices.
%
%\cite{l4} finds minimal corrective actions in response to transmission line failure. it also minimize the amount of redispatch power. Does not consider generator outages or reactive power limits. 
%
%\cite{l5, l7} solve SCOPF problem with convex relaxation approach. 
%
%\cite{l2}, \cite{l3}, \cite{l4} ignores reactive power limits. Also, they do not point out how to handle power mismatch or network losses.  
%
%\cite{l8} extends \cite{l7} to integrate optimize settings of load tap changers and shunt capacitor banks.
%
%
%none of the above-given paper integrates reactive power limits or bus type switching into its problem formulation.
%
%, , , offer different methods how to integrate QV modeling curve of generator. Since it is undifferentiable at the turning points where the newton method does not work. Therefore hyperbolic or sigmoid function is proposed to smooth the QV curve of generator.  

 

==> PV_PQ paper/nota.tex <==

\section{Notations and Power Grid Terminologies}
\subsection{Notations} 

Bold lowercase and uppercase letters (e.g., $\abf,~ \Abf$) represent vectors and matrices, respectively. $\bm{1}$ and $\bm{0}$ refer to vectors with all elements as 1 and 0, respectively. The sets of complex and real numbers are shown with $\Cbb$ and $\Rbb$, respectively. $\Hbb^n$ and $\Sbb^n$ represent the hermitian and symmetric matrices of size $n \times n$, respectively. $\mathrm{imag}\{\cdot\}$ and $\mathrm{real}\{\cdot\}$ define the imaginary and real parts of a complex matrix or number, respectively. Superscripts $\!(\cdot)^{\!\top}\!$ and $\!(\cdot)^{\!\ast}\!$ stand for the transpose and conjugate transpose operator, respectively.  $|\cdot|$ represents the cardinality of a set or the absolute/magnitude value of a vector/scalar. 
$\diagrm\{\cdot\}$ forms a vector  using diagonal entries of a given matrix. $[\cdot]$ composes a diagonal matrix from a given vector. 
  \begin{figure} 
 	\centering  
 	\includegraphics[width=\columnwidth]{figures/fig1.pdf}
 	\caption{Contingency scenario examples for a portion of the power grid. The base case refers to the scenario 0, i.e., no contingency. The red labels highlight the failure of a generator and a transmission line. In Scenario 1, generator 1 fails while generator 2 readjusts its output according to weight $\alpha_{1,2}$. Scenario 2 illustrates a transmission line failure, while generators 1 and 2 contribute to the power re-dispatch $\Delta_2$.}
 	\label{fig:1}
 \end{figure}
 \subsection{Power Grid Terminologies} 
 
Figure~\ref{fig:1} shows a snapshot of a power grid, where any single bus can accommodate an arbitrary number of generators and loads. The set of contingency scenarios is referred to as $\Ccal$, with each positive member accounting for the outage of, at least, one network component, e.g., a generator or a transmission line. Herein, the \textit{base case scenario}, i.e., normal operation with no contingency, is shown by $0 \in \Ccal$. For the rest of the scenarios, $c \in \Ccal$, grid terminologies are detailed as:
\begin{itemize}
\item {\bf Buses and Lines:} The transmission grid is structured using a directed graph $\Hcal=\left(\Ncal,\Lcal\right)$, where  the sets of buses and lines are denoted by $\Ncal$ and $\Lcal$, respectively. Let   $\vec{\Lbf}_c,\cev{\Lbf}_c\in\{0,1\}^{|\Lcal|\times|\Ncal|}$  be the pairs for the {\it from} and {\it to} line-incidence matrices in a contingency case, respectively. $\vec{L}_{c,_{li}} = 1$ and $\cev{L}_{c,_{li}}=1$ for every $l\in\mathcal{L}$, iff the transmission line $l$ starts at bus $i$, and vice versa, respectively. Matrices $\Ybf_c \in \Cbb^{|\Ncal| \times |\Ncal|}$, $\vec{\Ybf}_c,\cev{\Ybf}_c \in \Cbb^{|\Lcal| \times |\Ncal|}$ respectively denote the bus-admittance, and the {\it from} and {\it to} line-admittance matrices (See \cite{zimmerman2016matpower} for the definition of admittance matrices). Let $\sbf^{\rm{max}}_c\in(\Cbb\cup\{\infty\})^{|\Lcal|}$ be the vector of apparent power flow limits on transmission lines. Define $\vbf_0$, $\vbf_c \in \Cbb^{|\Ncal|}$ as the vectors of complex nodal voltages in the base and contingency cases, respectively. Define $\vbf^{\rm{max}},\vbf^{\rm{min}}\in\Cbb^{|\Ncal|}$ as the vectors of the maximum and minimum voltage magnitudes, respectively.
\item {\bf Generators/Loads:} 
Let $\Gcal$ be the set of generators and $\Gbf_c \in \{0,1\}^{|\Gcal|\times|\Ncal|}$ as the generator incidence matrix in a contingency case; $(g,i)$ element is $1$ iff generator $g\in \Gcal$ is located at the bus $i\in \Ncal$ and not outed in the event of contingency $c$.   $\Cbf_c \in \{0,1\}^{|\Gcal|\times|\Gcal|}$ denotes a diagonal incidence matrix whose $(g,g)$ element is $1$, iff the generator $g\in\Gcal$ is in service in the event of contingency $c$.  $\sbf^{\rm{dem}}_c\in\Cbb$ represents the vectors of apparent power demand. Let $\sbf^{\rm{gen}}_0\in\Cbb^{|\Gcal|}$, and $\pbf^{\rm{gen}}_0,\qbf^{\rm{gen}}_0\in\Rbb^{|\Gcal|}$, respectively, represent the vectors of apparent, active, and reactive power generations in the base case, while for every $c\in\Ccal$ $\sbf^{\rm{gen}}_c\in\Cbb^{|\Gcal|}$, and $\pbf^{\rm{gen}}_c,\qbf^{\rm{gen}}_c\in\Rbb^{|\Gcal|}$ represent the corresponding post-contingency power generation vectors. Define $\pbf^{\rm{max}}_c,\qbf^{\rm{max}}_c\in\Rbb^{|\Gcal|}$
and $\pbf^{\rm{min}}_c,\qbf^{\rm{min}}_c\in\Rbb^{|\Gcal|}$ as the vectors of the maximum and minimum active and reactive power generations, respectively.

	
\end{itemize}	

==> PV_PQ paper/notations.tex <==
\newcommand{\st}{\mathrm{subject~to}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\onebf}{\boldsymbol{1}}

\newcommand{\abf}{\boldsymbol{a}}
\newcommand{\Abf}{\boldsymbol{A}}
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}

\newcommand{\bbf}{\boldsymbol{b}}
\newcommand{\Bbf}{\boldsymbol{B}}
\newcommand{\Bcal}{\mathcal{B}}

\newcommand{\Cbf}{\boldsymbol{C}}
\newcommand{\cbf}{\boldsymbol{c}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Cbb}{\mathbb{C}}

\newcommand{\dbf}{\boldsymbol{d}}
\newcommand{\Dbf}{\boldsymbol{D}}
\newcommand{\Dcal}{\mathcal{D}}

\newcommand{\ebf}{\boldsymbol{e}}
\newcommand{\Ebf}{\boldsymbol{E}}
\newcommand{\Ecal}{\mathcal{E}}

\newcommand{\fbf}{\boldsymbol{f}}
\newcommand{\Fbf}{\boldsymbol{F}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\frm}{\mathrm{f}}

\newcommand{\gbf}{\boldsymbol{g}}
\newcommand{\Gbf}{\boldsymbol{G}}
\newcommand{\Gcal}{\mathcal{G}}

\newcommand{\hbf}{\boldsymbol{h}}
\newcommand{\Hbf}{\boldsymbol{H}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Hbb}{\mathbb{H}}

\newcommand{\ibf}{\boldsymbol{i}}
\newcommand{\Ibf}{\boldsymbol{I}}
\newcommand{\irm}{\mathrm{i}}

\newcommand{\jbf}{\boldsymbol{j}}
\newcommand{\Jbf}{\boldsymbol{J}}
\newcommand{\Jcal}{\mathcal{J}}

\newcommand{\kbf}{\boldsymbol{k}}
\newcommand{\Kbf}{\boldsymbol{K}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Krm}{\mathrm{K}}

\newcommand{\lbf}{\boldsymbol{l}}
\newcommand{\Lbf}{\boldsymbol{L}}
\newcommand{\Lcal}{\mathcal{L}}

\newcommand{\mbf}{\boldsymbol{m}}
\newcommand{\Mbf}{\boldsymbol{M}}
\newcommand{\mrm}{\mathrm{m}}
\newcommand{\Mcal}{\mathcal{M}}

\newcommand{\nbf}{\boldsymbol{n}}
\newcommand{\Nbf}{\boldsymbol{N}}
\newcommand{\Ncal}{\mathcal{N}}

\newcommand{\Ob}{\boldsymbol{O}}
\newcommand{\obf}{\boldsymbol{o}}

\newcommand{\pbf}{\boldsymbol{p}}
\newcommand{\Pbf}{\boldsymbol{P}}
\newcommand{\Pcal}{\mathcal{P}}

\newcommand{\qbf}{\boldsymbol{q}}
\newcommand{\Qbf}{\boldsymbol{Q}}

\newcommand{\rbf}{\boldsymbol{r}}
\newcommand{\Rbf}{\boldsymbol{R}}
\newcommand{\rrm}{\mathrm{r}}
\newcommand{\Rbb}{\mathbb{R}}
\newcommand{\Rcal}{\mathcal{R}}

\newcommand{\sbf}{\boldsymbol{s}}
\newcommand{\Sbf}{\boldsymbol{S}}
\newcommand{\Sbb}{\mathbb{S}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Zcal}{\mathcal{Z}}

\newcommand{\tbf}{\boldsymbol{t}}
\newcommand{\Tbf}{\boldsymbol{T}}
\newcommand{\trm}{\mathrm{t}}

\newcommand{\ubf}{\boldsymbol{u}}
\newcommand{\Ubf}{\boldsymbol{U}}

\newcommand{\vbf}{\boldsymbol{v}}
\newcommand{\Vbf}{\boldsymbol{V}}
\newcommand{\Vcal}{\mathcal{V}}

\newcommand{\wbf}{\boldsymbol{w}}
\newcommand{\Wbf}{\boldsymbol{W}}

\newcommand{\xbf}{\boldsymbol{x}}
\newcommand{\Xbf}{\boldsymbol{X}}

\newcommand{\ybf}{\boldsymbol{y}}
\newcommand{\Ybf}{\boldsymbol{Y}}

\newcommand{\zbf}{\boldsymbol{z}}
\newcommand{\Zbf}{\boldsymbol{Z}}

\newcommand{\lambdabf}{\boldsymbol{\lambda}}
\newcommand{\gammabf}{\boldsymbol{\gamma}}
\newcommand{\betabf}{\boldsymbol{\beta}}
\newcommand{\alphabf}{\boldsymbol{\alpha}}
\newcommand{\etabf}{\boldsymbol{\eta}}
\newcommand{\mubf}{\boldsymbol{\mu}}
\newcommand{\deltabf}{\boldsymbol{\delta}}
\newcommand{\nubf}{\boldsymbol{\nu}}
\newcommand{\kappabf}{\boldsymbol{\kappa}}

\newcommand{\diagrm}{\mathrm{diag}}
\newcommand{\realrm}{\mathrm{real}}
\newcommand{\imagrm}{\mathrm{imag}}
\newcommand{\Rerm}{\mathrm{Re}}
\newcommand{\Imrm}{\mathrm{Im}}
\newcommand{\rankrm}{\mathrm{rank}}
\newcommand{\shrm}{\mathrm{sh}}
\newcommand{\maxrm}{\textnormal{max}}
\newcommand{\minrm}{\textnormal{min}}

\makeatletter
\DeclareRobustCommand{\cev}[1]{%
  \mathpalette\do@cev{#1}%
}
\newcommand{\do@cev}[2]{%
  \fix@cev{#1}{+}%
  \reflectbox{$\m@th#1\vec{\reflectbox{$\fix@cev{#1}{-}\m@th#1#2\fix@cev{#1}{+}$}}$}%
  \fix@cev{#1}{-}%
}
\newcommand{\fix@cev}[2]{%
  \ifx#1\displaystyle
    \mkern#2 1mu
  \else
    \ifx#1\textstyle
      \mkern#2 3mu
    \else
      \ifx#1\scriptstyle
        \mkern#2 2mu
      \else
        \mkern#2 2mu
      \fi
    \fi
  \fi
}
\newcommand{\cevhat}[1]{\hat{\reflectbox{\ensuremath{\vec{\ensuremath{#1}}}}}}
\newcommand{\cevstar}[1]{\accentset{\ast}{\reflectbox{\ensuremath{\vec{\ensuremath{#1}}}}}}

\def\vecsign{\mathchar"017E}
\def\dvecsign{\smash{\stackon[-1.95pt]{\vecsign}{\hspace{+1.0mm}\rotatebox{180}{$\vecsign$}}}}
\def\dvec#1{\def\useanchorwidth{T}\stackon[-4.2pt]{#1}{\hspace{-0.25mm}\dvecsign}}
\usepackage{stackengine}
\stackMath



==> PV_PQ paper/tablees.tex <==
\begin{table}[h]
\caption{Converter output Power results from optimization Fig1}
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Sc./ & 1 & 2 & 3 & 4 & 5\\
Bus &  &  &  & & \\
\hline
 1& 332.4 & 265.92  &299.16 &  332.4  & 365.64\\
 \hline
 2& 118.7 & 111.67 & 114.98 & 118.70 & 122.81\\
\hline
 3& 100 & 80 & 90 & 100 & 110\\
\hline
 6& 100 & 80 & 90 & 100 & 110\\
\hline
 8& 100 & 80 & 90 & 100 & 110\\
\hline
\end{tabular}
\end{table}
 
\begin{table}[h]
\caption{ Output Voltage results from optimization. Fig2,3}
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Sc./ & 1 & 2 & 3 & 4 & 5\\
Bus &  &  &  & & \\
\hline
 1& 49.70 & 48.84 & 49.27 &  49.70  & 50.12\\
 \hline
 2& 48.86 & 48.19 & 48.52 & 48.86 & 49.20\\
\hline
 3& 48.13 & 47.51 & 47.82 & 48.13 & 48.43\\
\hline
 4& 47.26 & 46.83 & 47.04 & 47.26 & 47.47\\
\hline
 5& 46.88 & 46.54 & 46.71 & 46.88 & 47.05\\
\hline
 6& 45.72 & 45.60 & 45.66 &  45.72  & 45.78\\
 \hline
 7& 47.35 & 46.90 & 47.12 & 47.35 & 47.57\\
\hline
 8& 47.75 & 47.21 & 47.48 & 47.75 & 48.02\\
\hline
 9& 47.04 & 46.66 & 46.85 & 47.04 & 47.23\\
\hline
 10& 46.84 & 46.50 & 46.67 & 46.84 & 47.01\\
\hline
 11& 46.32 & 46.08 & 46.20 &  46.32  & 46.44\\
 \hline
 12& 45.12 & 45.12 & 45.12 & 45.12 & 45.12\\
\hline
 13& 45.49 & 45.42 & 45.45 & 45.49 & 45.53\\
\hline
 14& 45.19 & 45.18 & 45.18 & 45.19 & 45.20\\
\hline
\end{tabular}
\end{table}   

\begin{table}[h]
\caption{Resistive Power results from optimization Fig5 }
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Sc./ & 1 & 2 & 3 & 4 & 5\\
Bus &  &  &  & & \\
\hline
 1& 18.11 &  17.49 &  17.80  & 18.11 &  18.43\\
 \hline
 2& 43.94  & 42.73  & 43.33 &   43.94 &  44.56\\
\hline
 3& 23.52  & 22.93  & 23.23  & 23.52 &  23.82\\
\hline
 6& 11.07  & 11.01  & 11.04 &  11.07 &  11.10\\
\hline
 8& 17.22 &  16.83 &  17.02  & 17.22 &  17.41\\
\hline
\end{tabular}
\end{table}   
   
\begin{table}[t]
\caption{Constant Power results from optimization Fig4}
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Sc./ & 1 & 2 & 3 & 4 & 5\\
Bus &  &  &  & & \\
\hline
 1&  109.00 &  87.20 &  98.10 & 109.00 & 119.90\\
 \hline
 3&  82.00 &  65.60 &  73.80 &  82.00 &  90.20\\
\hline
 6&  314.00 & 251.20 & 282.60 & 314.00 & 345.40\\
\hline
 9& 64.00  & 51.20 &  57.60 &  64.00 &  70.40\\
\hline
 12& 13.00 &  10.40  & 11.70  & 13.00 &  14.30\\
\hline
 14& 32.00 &  25.60 &  28.80 &  32.00 &  35.20\\
\hline
\end{tabular}
\end{table}  

\begin{table}[h]
\caption{Converter output Power results from optimization Fig6  (Load Shedding Active)}
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Sc./ & 1 & 2 & 3 & 4 & 5\\
Bus &  &  &  & & \\
\hline
 1& 189.63 & 263.43  &247.57  &   189.60  &  190.65\\
 \hline
 2& 35.96 & 47.92  & 46.25 & 35.96 & 36.16\\
\hline
 3& 38.22  & 80.00  & 90.00 & 38.23 & 44.27\\
\hline
 6& 2.76 & 80.00 & 90.00 & 2.76 & 7.61\\
\hline
 8& 3.83 & 80.00 & 90.00 & 3.84 & 7.97\\
\hline
\end{tabular}
\end{table}
       
  \begin{table}[h]
\caption{ Output Voltage results from optimization.Fig7-8(Load Shedding Active) }
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Sc./ & 1 & 2 & 3 & 4 & 5\\
Bus &  &  &  & & \\
\hline
 1& 47.45  & 48.77 &  49.44  & 47.45 &  47.49\\
 \hline
 2&  46.40 &  48.12  & 48.34 &  46.39 &  46.43\\
\hline
 3&  45.12 &  47.79 &  48.02 &  45.12 &  45.12\\
\hline
 4& 45.50  & 46.86 &  47.04 &  45.50 &  45.52\\
\hline
 5& 45.84 &  46.53  & 46.71 &  45.84 &  45.88\\
\hline
 6& 45.70 &  45.60 &  45.66 &  45.70 &  45.76\\
 \hline
 7& 45.36  & 46.92  & 47.12  & 45.36  & 45.39\\
\hline
 8& 45.30 &  47.23  & 47.48  & 45.30 &  45.35\\
\hline
 9& 45.28 &  46.68  & 46.85  & 45.28 &  45.29\\
\hline
 10& 45.34 &  46.52 &  46.67 &  45.34 &  45.36\\
\hline
 11& 45.51 &  46.09  & 46.20  & 45.51  & 45.55\\
 \hline
 12& 45.12 &  45.12 &  45.12 &  45.12 &  45.12\\
\hline
 13& 45.53 &  45.42 &  45.45 &  45.53  & 45.57\\
\hline
 14& 45.38 &  45.19  & 45.18  & 45.38 &  45.41\\
\hline
\end{tabular}
\end{table}
   
\begin{table}[h]
\caption{Resistive Power results from optimization Fig10  (Load Shedding Active)}
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Sc./ & 1 & 2 & 3 & 4 & 5\\
Bus &  &  &  & & \\
\hline
 1& 16.51  & 17.45 &  17.93 &  16.51  & 16.54\\
 \hline
 2& 39.62   &      0  & 43.02 &  39.62 &  39.67\\
\hline
 3& 20.67  &       0     &    0  & 20.67  & 20.67\\
\hline
 6& 11.06 &  11.01  & 11.04 &  11.06  & 11.09\\
\hline
 8& 15.49  & 16.85  & 17.02 &  15.49  & 15.53\\
\hline
\end{tabular}
\end{table}   
   
\begin{table}[h]
\caption{Constant Power results from optimization Fig9  (Load Shedding Active)}
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Sc./ & 1 & 2 & 3 & 4 & 5\\
Bus &  &  &  & & \\
\hline
 1&  0  & 87.2  & 0  &  0   &      0\\
 \hline
 3& 82.0 &  65.6 &  73.8  & 82.0&  90.2\\
\hline
 6&  0 & 251.2 &282.6&    0  &  0\\
\hline
 9& 64.0 &  51.2 &  57.6 &  64.0  & 70.4\\
\hline
 12& 13.0 & 10.4  & 11.7 &  13.0  & 14.3\\
\hline
 14& 0  & 25.6 & 28.8   &      0    &     0\\
\hline
\end{tabular}
\end{table}    

\begin{table}[h]
\caption{Converter output Power results from optimization Fig11  (Generator Commitment Active)}
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Sc./ & 1 & 2 & 3 & 4 & 5\\
Bus &  &  &  & & \\
\hline
 1&   198.82 & 261.22&  299.15 & 203.20 & 201.57\\
 \hline
 2&   37.70  & 49.45 &  58.37 &  39.03 &  38.27\\
\hline
 3&  0.00  &  0.00  &  0.00 &   0.00  &  0.00\\
\hline
 6& 31.01 &  80.00  & 90.00  &       0 &  39.89\\
\hline
 8& 41.69 & 79.99 &  90.00 &  32.26 &  50.12\\
\hline
\end{tabular}
\end{table}
      
\begin{table}[h]
\caption{ Output Voltage results from optimization.Fig 12-13(Generator Commitment Active) }
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Sc./ & 1 & 2 & 3 & 4 & 5\\
Bus &  &  &  & & \\
\hline
 1& 48.40 &  49.37 &  49.56  & 48.03 &  48.54\\
 \hline
 2&  47.27 &  48.18  & 48.11 &  46.88 &  47.38\\
\hline
 3&  45.52 &  46.69  & 46.56 &  45.12 &  45.52\\
\hline
 4& 46.52 &  46.73 &  46.80 &  46.11  & 46.65\\
\hline
 5& 46.89 &  46.55  & 46.56 &   46.42  & 47.04\\
\hline
 6& 46.83 &  45.61 &  45.56 &  46.28 &  47.01\\
 \hline
 7& 46.47 &  46.80 &  46.91 &  46.07 & 46.61\\
\hline
 8& 46.60 &  47.11 &  47.27 &  46.15 &  46.78\\
\hline
 9& 46.30 &  46.56 &  46.67 &  45.94 &  46.42\\
\hline
 10& 46.38 &  46.42 &  46.50 &  45.99 &  46.51\\
\hline
 11& 46.59 &  46.04 &  46.06 &  46.12 &  46.74\\
 \hline
 12& 46.13 &  45.12 &  45.12 &  45.70 &  46.24\\
\hline
 13& 46.31 &  45.41 &  45.63 &  46.12 &  46.44\\
\hline
 14& 45.12 &  45.12 &  46.23 &  46.01 &  45.12\\
\hline
\end{tabular}
\end{table}
 
\begin{table}[h]
\caption{Resistive Power results from optimization Fig15  (Generator Commitment Active)}
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Sc./ & 1 & 2 & 3 & 4 & 5\\
Bus &  &  &  & & \\
\hline
 1& 17.18&   17.88 &  18.02  & 16.92 &  17.28\\
 \hline
 2& 41.12   &      0 &  42.59 &  40.45 &  41.32\\
\hline
 3& 21.04   &      0    &     0 &  20.67 &  21.05\\
\hline
 6& 11.61  & 11.01 &  10.99  & 11.34 &  11.70\\
\hline
 8& 16.40 &  16.76 &  16.87  & 16.08 &  16.53\\
\hline
\end{tabular}
\end{table}   
 
\begin{table}[h]
\caption{Constant Power results from optimization Fig14  (Generator Commitment Active)}
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Sc./ & 1 & 2 & 3 & 4 & 5\\
Bus &  &  &  & & \\
\hline
 1&  0.00 &   0.00  &  0.00  &  0.00  &  0.00\\
 \hline
 3& 82.0 &  65.6 &  73.8  & 82.0&  90.2\\
\hline
 6&  0 & 251.20 &282.60&    0  &  0\\
\hline
 9& 64.0 &  51.20 &  57.60 &  64.00  & 70.40\\
\hline
 12& 13.0 & 10.40  & 11.70 &  13.00  & 14.30\\
\hline
 14& 32.00 &  25.60  &    0  &     0 &  35.20\\
\hline
\end{tabular}
\end{table}    

==> tablees.tex <==
\begin{table}[h]
\caption{Converter output Power results from optimization Fig1}
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Sc./ & 1 & 2 & 3 & 4 & 5\\
Bus &  &  &  & & \\
\hline
 1& 332.4 & 265.92  &299.16 &  332.4  & 365.64\\
 \hline
 2& 118.7 & 111.67 & 114.98 & 118.70 & 122.81\\
\hline
 3& 100 & 80 & 90 & 100 & 110\\
\hline
 6& 100 & 80 & 90 & 100 & 110\\
\hline
 8& 100 & 80 & 90 & 100 & 110\\
\hline
\end{tabular}
\end{table}
 
\begin{table}[h]
\caption{ Output Voltage results from optimization. Fig2,3}
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Sc./ & 1 & 2 & 3 & 4 & 5\\
Bus &  &  &  & & \\
\hline
 1& 49.70 & 48.84 & 49.27 &  49.70  & 50.12\\
 \hline
 2& 48.86 & 48.19 & 48.52 & 48.86 & 49.20\\
\hline
 3& 48.13 & 47.51 & 47.82 & 48.13 & 48.43\\
\hline
 4& 47.26 & 46.83 & 47.04 & 47.26 & 47.47\\
\hline
 5& 46.88 & 46.54 & 46.71 & 46.88 & 47.05\\
\hline
 6& 45.72 & 45.60 & 45.66 &  45.72  & 45.78\\
 \hline
 7& 47.35 & 46.90 & 47.12 & 47.35 & 47.57\\
\hline
 8& 47.75 & 47.21 & 47.48 & 47.75 & 48.02\\
\hline
 9& 47.04 & 46.66 & 46.85 & 47.04 & 47.23\\
\hline
 10& 46.84 & 46.50 & 46.67 & 46.84 & 47.01\\
\hline
 11& 46.32 & 46.08 & 46.20 &  46.32  & 46.44\\
 \hline
 12& 45.12 & 45.12 & 45.12 & 45.12 & 45.12\\
\hline
 13& 45.49 & 45.42 & 45.45 & 45.49 & 45.53\\
\hline
 14& 45.19 & 45.18 & 45.18 & 45.19 & 45.20\\
\hline
\end{tabular}
\end{table}   

\begin{table}[h]
\caption{Resistive Power results from optimization Fig5 }
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Sc./ & 1 & 2 & 3 & 4 & 5\\
Bus &  &  &  & & \\
\hline
 1& 18.11 &  17.49 &  17.80  & 18.11 &  18.43\\
 \hline
 2& 43.94  & 42.73  & 43.33 &   43.94 &  44.56\\
\hline
 3& 23.52  & 22.93  & 23.23  & 23.52 &  23.82\\
\hline
 6& 11.07  & 11.01  & 11.04 &  11.07 &  11.10\\
\hline
 8& 17.22 &  16.83 &  17.02  & 17.22 &  17.41\\
\hline
\end{tabular}
\end{table}   
   
\begin{table}[t]
\caption{Constant Power results from optimization Fig4}
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Sc./ & 1 & 2 & 3 & 4 & 5\\
Bus &  &  &  & & \\
\hline
 1&  109.00 &  87.20 &  98.10 & 109.00 & 119.90\\
 \hline
 3&  82.00 &  65.60 &  73.80 &  82.00 &  90.20\\
\hline
 6&  314.00 & 251.20 & 282.60 & 314.00 & 345.40\\
\hline
 9& 64.00  & 51.20 &  57.60 &  64.00 &  70.40\\
\hline
 12& 13.00 &  10.40  & 11.70  & 13.00 &  14.30\\
\hline
 14& 32.00 &  25.60 &  28.80 &  32.00 &  35.20\\
\hline
\end{tabular}
\end{table}  

\begin{table}[h]
\caption{Converter output Power results from optimization Fig6  (Load Shedding Active)}
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Sc./ & 1 & 2 & 3 & 4 & 5\\
Bus &  &  &  & & \\
\hline
 1& 189.63 & 263.43  &247.57  &   189.60  &  190.65\\
 \hline
 2& 35.96 & 47.92  & 46.25 & 35.96 & 36.16\\
\hline
 3& 38.22  & 80.00  & 90.00 & 38.23 & 44.27\\
\hline
 6& 2.76 & 80.00 & 90.00 & 2.76 & 7.61\\
\hline
 8& 3.83 & 80.00 & 90.00 & 3.84 & 7.97\\
\hline
\end{tabular}
\end{table}
       
  \begin{table}[h]
\caption{ Output Voltage results from optimization.Fig7-8(Load Shedding Active) }
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Sc./ & 1 & 2 & 3 & 4 & 5\\
Bus &  &  &  & & \\
\hline
 1& 47.45  & 48.77 &  49.44  & 47.45 &  47.49\\
 \hline
 2&  46.40 &  48.12  & 48.34 &  46.39 &  46.43\\
\hline
 3&  45.12 &  47.79 &  48.02 &  45.12 &  45.12\\
\hline
 4& 45.50  & 46.86 &  47.04 &  45.50 &  45.52\\
\hline
 5& 45.84 &  46.53  & 46.71 &  45.84 &  45.88\\
\hline
 6& 45.70 &  45.60 &  45.66 &  45.70 &  45.76\\
 \hline
 7& 45.36  & 46.92  & 47.12  & 45.36  & 45.39\\
\hline
 8& 45.30 &  47.23  & 47.48  & 45.30 &  45.35\\
\hline
 9& 45.28 &  46.68  & 46.85  & 45.28 &  45.29\\
\hline
 10& 45.34 &  46.52 &  46.67 &  45.34 &  45.36\\
\hline
 11& 45.51 &  46.09  & 46.20  & 45.51  & 45.55\\
 \hline
 12& 45.12 &  45.12 &  45.12 &  45.12 &  45.12\\
\hline
 13& 45.53 &  45.42 &  45.45 &  45.53  & 45.57\\
\hline
 14& 45.38 &  45.19  & 45.18  & 45.38 &  45.41\\
\hline
\end{tabular}
\end{table}
   
\begin{table}[h]
\caption{Resistive Power results from optimization Fig10  (Load Shedding Active)}
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Sc./ & 1 & 2 & 3 & 4 & 5\\
Bus &  &  &  & & \\
\hline
 1& 16.51  & 17.45 &  17.93 &  16.51  & 16.54\\
 \hline
 2& 39.62   &      0  & 43.02 &  39.62 &  39.67\\
\hline
 3& 20.67  &       0     &    0  & 20.67  & 20.67\\
\hline
 6& 11.06 &  11.01  & 11.04 &  11.06  & 11.09\\
\hline
 8& 15.49  & 16.85  & 17.02 &  15.49  & 15.53\\
\hline
\end{tabular}
\end{table}   
   
\begin{table}[h]
\caption{Constant Power results from optimization Fig9  (Load Shedding Active)}
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Sc./ & 1 & 2 & 3 & 4 & 5\\
Bus &  &  &  & & \\
\hline
 1&  0  & 87.2  & 0  &  0   &      0\\
 \hline
 3& 82.0 &  65.6 &  73.8  & 82.0&  90.2\\
\hline
 6&  0 & 251.2 &282.6&    0  &  0\\
\hline
 9& 64.0 &  51.2 &  57.6 &  64.0  & 70.4\\
\hline
 12& 13.0 & 10.4  & 11.7 &  13.0  & 14.3\\
\hline
 14& 0  & 25.6 & 28.8   &      0    &     0\\
\hline
\end{tabular}
\end{table}    

\begin{table}[h]
\caption{Converter output Power results from optimization Fig11  (Generator Commitment Active)}
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Sc./ & 1 & 2 & 3 & 4 & 5\\
Bus &  &  &  & & \\
\hline
 1&   198.82 & 261.22&  299.15 & 203.20 & 201.57\\
 \hline
 2&   37.70  & 49.45 &  58.37 &  39.03 &  38.27\\
\hline
 3&  0.00  &  0.00  &  0.00 &   0.00  &  0.00\\
\hline
 6& 31.01 &  80.00  & 90.00  &       0 &  39.89\\
\hline
 8& 41.69 & 79.99 &  90.00 &  32.26 &  50.12\\
\hline
\end{tabular}
\end{table}
      
\begin{table}[h]
\caption{ Output Voltage results from optimization.Fig 12-13(Generator Commitment Active) }
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Sc./ & 1 & 2 & 3 & 4 & 5\\
Bus &  &  &  & & \\
\hline
 1& 48.40 &  49.37 &  49.56  & 48.03 &  48.54\\
 \hline
 2&  47.27 &  48.18  & 48.11 &  46.88 &  47.38\\
\hline
 3&  45.52 &  46.69  & 46.56 &  45.12 &  45.52\\
\hline
 4& 46.52 &  46.73 &  46.80 &  46.11  & 46.65\\
\hline
 5& 46.89 &  46.55  & 46.56 &   46.42  & 47.04\\
\hline
 6& 46.83 &  45.61 &  45.56 &  46.28 &  47.01\\
 \hline
 7& 46.47 &  46.80 &  46.91 &  46.07 & 46.61\\
\hline
 8& 46.60 &  47.11 &  47.27 &  46.15 &  46.78\\
\hline
 9& 46.30 &  46.56 &  46.67 &  45.94 &  46.42\\
\hline
 10& 46.38 &  46.42 &  46.50 &  45.99 &  46.51\\
\hline
 11& 46.59 &  46.04 &  46.06 &  46.12 &  46.74\\
 \hline
 12& 46.13 &  45.12 &  45.12 &  45.70 &  46.24\\
\hline
 13& 46.31 &  45.41 &  45.63 &  46.12 &  46.44\\
\hline
 14& 45.12 &  45.12 &  46.23 &  46.01 &  45.12\\
\hline
\end{tabular}
\end{table}
 
\begin{table}[h]
\caption{Resistive Power results from optimization Fig15  (Generator Commitment Active)}
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Sc./ & 1 & 2 & 3 & 4 & 5\\
Bus &  &  &  & & \\
\hline
 1& 17.18&   17.88 &  18.02  & 16.92 &  17.28\\
 \hline
 2& 41.12   &      0 &  42.59 &  40.45 &  41.32\\
\hline
 3& 21.04   &      0    &     0 &  20.67 &  21.05\\
\hline
 6& 11.61  & 11.01 &  10.99  & 11.34 &  11.70\\
\hline
 8& 16.40 &  16.76 &  16.87  & 16.08 &  16.53\\
\hline
\end{tabular}
\end{table}   
 
\begin{table}[h]
\caption{Constant Power results from optimization Fig14  (Generator Commitment Active)}
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Sc./ & 1 & 2 & 3 & 4 & 5\\
Bus &  &  &  & & \\
\hline
 1&  0.00 &   0.00  &  0.00  &  0.00  &  0.00\\
 \hline
 3& 82.0 &  65.6 &  73.8  & 82.0&  90.2\\
\hline
 6&  0 & 251.20 &282.60&    0  &  0\\
\hline
 9& 64.0 &  51.20 &  57.60 &  64.00  & 70.40\\
\hline
 12& 13.0 & 10.40  & 11.70 &  13.00  & 14.30\\
\hline
 14& 32.00 &  25.60  &    0  &     0 &  35.20\\
\hline
\end{tabular}
\end{table}    
